Rethinking Multi-domain Generalization with A General Learning Objective

Multi-domain generalization (mDG) is universally aimed to minimize the discrepancy between training and testing distributions to enhance marginal-to-label distribution mapping. However, existing mDG literature lacks a general learning objective paradigm and often imposes constraints on static target marginal distributions. In this paper, we propose to leverage a $Y$-mapping to relax the constraint. We rethink the learning objective for mDG and design a new \textbf{general learning objective} to interpret and analyze most existing mDG wisdom. This general objective is bifurcated into two synergistic amis: learning domain-independent conditional features and maximizing a posterior. Explorations also extend to two effective regularization terms that incorporate prior information and suppress invalid causality, alleviating the issues that come with relaxed constraints. We theoretically contribute an upper bound for the domain alignment of domain-independent conditional features, disclosing that many previous mDG endeavors actually \textbf{optimize partially the objective} and thus lead to limited performance. As such, our study distills a general learning objective into four practical components, providing a general, robust, and flexible mechanism to handle complex domain shifts. Extensive empirical results indicate that the proposed objective with $Y$-mapping leads to substantially better mDG performance in various downstream tasks, including regression, segmentation, and classification.

==> sup.tex <==
\clearpage
% \setcounter{page}{1}
\maketitlesupplementary


% \twocolumn[
% \begin{@twocolumnfalse}
% \section{Appendix}
% \begin{page*}



\section{More mathematical details of our method}
\label{app:our_obj}
\subsection{Derivation details of PUB}

\textbf{Details for Eq.~\ref{eq:bound1}.}

We denote $P_{mix} \triangleq \sum_n w_n P({\phi(\rmX_n), \psi(\rmY_n)}) $.  Therefore for GJSD, we have:
% \begin{align}
%      & GJSD(\{P ({\phi(\rmX_n), \psi(\rmY_n)})\}_{n=1}^{N}) 
%      \\ 
%      = &\sum\nolimits_n w_n KL (P(\phi(\rmX_n) ,  \psi(\rmY_n))\Vert P_{mix}) 
%      \nonumber \\
%      = &\sum\nolimits_n w_n [H_c( P(\phi(\rmX_n), \psi(\rmY_n)), P_{mix}) - H(P(\phi(\rmX_n), \psi(\rmY_n)))] 
%      \nonumber \\
%      = &\sum\nolimits_n w_n H_c( P(\phi(\rmX_n), \psi(\rmY_n)), P_{mix}) - \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n)))
%      \nonumber \\
%      = &\sum\nolimits_n w_n \int_{X,Y} - P(\phi(\rmX_n), \psi(\rmY_n))(x, y) \ln P_{mix}(x,y) d(x,y)  - \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n)))  
%      \nonumber \\
%      = &\int_{X,Y} - \sum\nolimits_n w_n P(\phi(\rmX_n), \psi(\rmY_n))(x, y) \ln P_{mix}(x,y) d(x,y) - \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))) 
%      \nonumber \\
%       = &\int_{X,Y} - P_{mix}(x,y) \ln P_{mix}(x,y) d(x,y) - \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))) 
%      \nonumber \\
%      = & H(P_{mix}) - \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))).
%      \nonumber
% \end{align}
% \begin{align}
%      & GJSD(\{P ({\phi(\rmX_n), \psi(\rmY_n)})\}_{n=1}^{N}) 
%      \\ 
%      = &\sum\nolimits_n w_n KL (P(\phi(\rmX_n) ,  \psi(\rmY_n))\Vert P_{mix}) 
%      \nonumber \\
%      = &\sum\nolimits_n w_n [H_c( P(\phi(\rmX_n), \psi(\rmY_n)), P_{mix}) \nonumber \\ 
%     &- H(P(\phi(\rmX_n), \psi(\rmY_n)))] 
%      \nonumber \\
%      = &\sum\nolimits_n w_n H_c( P(\phi(\rmX_n), \psi(\rmY_n)), P_{mix}) \nonumber \\ 
%     &- \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n)))
%      \nonumber \\
%      = &\sum\nolimits_n w_n \int_{\phi(\rmX_n), \psi(\rmY_n)} - P(x,y) \ln P_{mix}(x,y) d(x,y)  \nonumber \\ 
%     &- \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n)))  
%      \nonumber \\
%      = &\int_{\phi(\rmX_n), \psi(\rmY_n)} - \sum\nolimits_n w_n P(x, y) \ln P_{mix}(x,y) d(x,y) -\nonumber \\ 
%     & \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))) 
%      \nonumber \\
%       = &\int_{\phi(\rmX_n), \psi(\rmY_n)} - P_{mix}(x,y) \ln P_{mix}(x,y) d(x,y) \nonumber \\ 
%     &- \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))) 
%      \nonumber \\
%      = & H(P_{mix}) - \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))).
%      \nonumber
% \end{align}
\begin{equation}
    \begin{split}
             & GJSD(\{P ({\phi(\rmX_n), \psi(\rmY_n)})\}_{n=1}^{N}) 
     \\ 
     = &\sum\nolimits_n w_n KL (P(\phi(\rmX_n) ,  \psi(\rmY_n))\Vert P_{mix}) 
      \\
     = &\sum\nolimits_n w_n [H_c( P(\phi(\rmX_n), \psi(\rmY_n)), P_{mix})  \\ 
    &- H(P(\phi(\rmX_n), \psi(\rmY_n)))] 
      \\
     = &\sum\nolimits_n w_n H_c( P(\phi(\rmX_n), \psi(\rmY_n)), P_{mix})  \\ 
    &- \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n)))
      \\
     = &\sum\nolimits_n w_n \int_{\phi(\rmX_n), \psi(\rmY_n)} - P(x,y) \ln P_{mix}(x,y) d(x,y)   \\ 
    &- \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n)))  
      \\
     = &\int_{\phi(\rmX_n), \psi(\rmY_n)} - \sum\nolimits_n w_n P(x, y) \ln P_{mix}(x,y) d(x,y) \\ 
    & - \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))) 
      \\
      = &\int_{\phi(\rmX_n), \psi(\rmY_n)} - P_{mix}(x,y) \ln P_{mix}(x,y) d(x,y)  \\ 
    &- \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))) 
      \\
     = & H(P_{mix}) - \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))).
    \end{split}
\end{equation}


Therefore, the minimization of GJSD can be written as follows:
% \begin{align}
%     & \min_{\phi, \psi} GJSD(\{P ({\phi(\rmX_n), \psi(\rmY_n)})\}_{n=1}^{N}) 
%     \nonumber \\
%     \equiv &\min_{\phi, \psi} H(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})]) - \mathbb{E}[ H (P ({\phi(\rmX_n), \psi(\rmY_n)}))]\nonumber \\
%      \equiv &\min_{\phi, \psi}  H( P ({\phi(\rmX), \psi(\rmY)} \mid \mathcal{D})) - \mathbb{E} [H (P ({\phi(\rmX_n), \psi(\rmY_n)}))].\nonumber 
%      % = & H_c(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})],\mathcal{O})- \mathbb{E}[ H(P(\phi(\rmX_n), \psi(\rmY_n)))]
%      % \nonumber \\
%      %  = & H_c(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})],\mathcal{O})- a.
%      % \nonumber 
% \end{align}
\begin{equation}
    \resizebox{\hsize}{!}{$\begin{split}
    & \min_{\phi, \psi} GJSD(\{P ({\phi(\rmX_n), \psi(\rmY_n)})\}_{n=1}^{N}) 
     \\
    \equiv &\min_{\phi, \psi} H(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})]) - \mathbb{E}[ H (P ({\phi(\rmX_n), \psi(\rmY_n)}))] \\
     \equiv &\min_{\phi, \psi}  H( P ({\phi(\rmX), \psi(\rmY)} \mid \mathcal{D})) - \mathbb{E} [H (P ({\phi(\rmX_n), \psi(\rmY_n)}))]. 
     % = & H_c(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})],\mathcal{O})- \mathbb{E}[ H(P(\phi(\rmX_n), \psi(\rmY_n)))]
     % \nonumber \\
     %  = & H_c(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})],\mathcal{O})- a.
     % \nonumber 
    \end{split}$}
\end{equation}

% For the standard situation where $w_1 = w_2 = ... =  w_n = 1/N$, we further have:
% \begin{align}
%      & GJSD(\{P ({\phi(\rmX_n), \psi(\rmY_n)})\}_{n=1}^{N}) 
%      \\
%      = & H(P_{mix}) - \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))) 
%        \nonumber \\
%      = & H(\sum_n w_n P({\phi(\rmX_n), \psi(\rmY_n)})) - \sum\nolimits_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))) 
%      \nonumber 
%      % = & H(\mathbb{E}[ P({\phi(\rmX_n), \psi(\rmY_n)})]) - \mathbb{E}[ H(P(\phi(\rmX_n), \psi(\rmY_n)))].
%      % \nonumber
% \end{align}

\textbf{Details for Eq.~\ref{eq:bound2}.} Taking into account $\mathcal{O}$,  similar to \citep{cho2022cooperative}, we have the upper bound for GJSD as:
% \begin{align}
%      & GJSD(\{P ({\phi(\rmX_n), \psi(\rmY_n)})\}_{n=1}^{N}) 
%      \\ 
%      = & H_c(P_{mix}, \mathcal{O}) -   H_c(P_{mix}, \mathcal{O}) + H(P_{mix})  \nonumber \\ 
%     & -\sum_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))) 
%      \nonumber \\
%      = & H_c(P_{mix}, \mathcal{O}) - \KL( P_{mix} \Vert \mathcal{O}) \nonumber \\ 
%     & - \sum_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))) 
%      \nonumber \\
%      \leq & H_c(P_{mix}, \mathcal{O}) - \sum_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))). 
%      \nonumber
%      % = & H(P_{mix}) + \KL( P_{mix} \Vert \mathcal{O})  - \sum_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))).
%      % \nonumber
% \end{align}
\begin{equation}
    \begin{split}
         & GJSD(\{P ({\phi(\rmX_n), \psi(\rmY_n)})\}_{n=1}^{N}) 
     \\ 
     = & H_c(P_{mix}, \mathcal{O}) -   H_c(P_{mix}, \mathcal{O}) + H(P_{mix})   \\ 
    & -\sum_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))) 
      \\
     = & H_c(P_{mix}, \mathcal{O}) - \KL( P_{mix} \Vert \mathcal{O})  \\ 
    & - \sum_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))) 
      \\
     \leq & H_c(P_{mix}, \mathcal{O}) - \sum_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))). 
     % = & H(P_{mix}) + \KL( P_{mix} \Vert \mathcal{O})  - \sum_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))).
     % \nonumber
    \end{split}
\end{equation}
For the standard situation where $w_1 = w_2 = ... =  w_n = 1/N$, we further have:
% \begin{align}
%     & GJSD(\{P ({\phi(\rmX_n), \psi(\rmY_n)})\}_{n=1}^{N}) 
%     \nonumber \\
%      \leq & H_c(P_{mix}, \mathcal{O}) - \sum_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))) 
%      \nonumber \\
%      = & H_c(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})],\mathcal{O}) \\ 
%      &- \mathbb{E}[ H(P(\phi(\rmX_n), \psi(\rmY_n)))].
%      % \nonumber \\
%      %  = & H_c(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})],\mathcal{O})- a.
%      % \nonumber 
% \end{align}
\begin{equation}
    \begin{split}
        & GJSD(\{P ({\phi(\rmX_n), \psi(\rmY_n)})\}_{n=1}^{N}) 
     \\
     \leq & H_c(P_{mix}, \mathcal{O}) - \sum_n w_n H(P(\phi(\rmX_n), \psi(\rmY_n))) 
      \\
     = & H_c(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})],\mathcal{O}) \\ 
     &- \mathbb{E}[ H(P(\phi(\rmX_n), \psi(\rmY_n)))].
     % \nonumber \\
     %  = & H_c(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})],\mathcal{O})- a.
     % \nonumber 
    \end{split}
\end{equation}

\textbf{Details for Eq.~\ref{eq:PUB}.} The above bound can be further reformed as:
% \begin{align}
%      & H_c(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})],\mathcal{O})- a 
%      \nonumber \\
%        =  & H(\mathbb{E}  [P({\phi(\rmX_n), \psi(\rmY_n)})]) \nonumber \\ 
%     & + \KL(\mathbb{E}[P({\phi(\rmX_n), \psi(\rmY_n)})] \Vert \mathcal{O})  - a,
%         \nonumber \\
%       =  & H(\mathbb{E}  [P({\phi(\rmX_n), \psi(\rmY_n)})]) \nonumber \\ 
%     & + \KL(P({\phi(\rmX), \psi(\rmY)}) \Vert \mathcal{O})  - a.
% \end{align}
\begin{equation}
    \begin{split}
         & H_c(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})],\mathcal{O})- a 
      \\
       =  & H(\mathbb{E}  [P({\phi(\rmX_n), \psi(\rmY_n)})])  \\ 
    & + \KL(\mathbb{E}[P({\phi(\rmX_n), \psi(\rmY_n)})] \Vert \mathcal{O})  - a,
         \\
      =  & H(\mathbb{E}  [P({\phi(\rmX_n), \psi(\rmY_n)})])  \\ 
    & + \KL(P({\phi(\rmX), \psi(\rmY)}) \Vert \mathcal{O})  - a.
    \end{split}
\end{equation}
% where is the proposed PUB.


\textbf{Derivation details of Eq.~\ref{eq:GAim1_GReg2}.}
% \begin{align}
% %\label{eq:GAim1_GReg2}
%     \text{\textbf{GAim1}} = &H( P ({\phi(\rmX), \psi(\rmY)} \mid \mathcal{D})) \\
%      = & H(P (\phi(\rmX), \psi(\rmY), \mathcal{D})) -H(P(\mathcal{D}))\nonumber\\ 
%      = & H(P (\phi(\rmX), \mathcal{D})) - H(P(\mathcal{D})) \nonumber\\ & +  H(P(\psi(\rmY)\mid \phi(\rmX), \mathcal{D})) \nonumber\\ 
%     = & H(P (\phi(\rmX )\mid \mathcal{D})) +  H(P(\psi(\rmY)\mid \phi(\rmX), \mathcal{D})) \nonumber\\ 
%     = & H(P (\psi(\rmY)\mid \mathcal{D})) +  H(P(\phi(\rmX) \mid \psi(\rmY),  \mathcal{D})). \nonumber
%     % & - I(P (\phi(\rmX)); P(\psi(\rmY))\mid \mathcal{D}) \\
%     % \nonumber\\ 
%     % - I(P (\phi(\rmX)); P(\psi(\rmY))\mid \mathcal{D}) & = - I(X,Y;D) \\
%     % \text{\textbf{GReg2}} = & {\min_{\phi,\psi} - H(P(\phi(\rmX)  \mid  \psi(\rmY))) +H(P(\phi(\rmX)))}
%     % \\
%     % = & {\min_{\phi,\psi}I( P (\phi(\rmX)); P(\psi(\rmY))) 
% \end{align}
\begin{equation}
    \begin{split}
     \text{\textbf{GAim1}} = &H( P ({\phi(\rmX), \psi(\rmY)} \mid \mathcal{D})) \\
     = & H(P (\phi(\rmX), \psi(\rmY), \mathcal{D})) -H(P(\mathcal{D}))\\ 
     = & H(P (\phi(\rmX), \mathcal{D})) - H(P(\mathcal{D})) \\ & +  H(P(\psi(\rmY)\mid \phi(\rmX), \mathcal{D})) \\ 
    = & H(P (\phi(\rmX )\mid \mathcal{D})) +  H(P(\psi(\rmY)\mid \phi(\rmX), \mathcal{D})) \\ 
    = & H(P (\psi(\rmY)\mid \mathcal{D})) +  H(P(\phi(\rmX) \mid \psi(\rmY),  \mathcal{D})). 
    \end{split}
\end{equation}


\textbf{Derivation details of Eq.~\ref{eq:why_greg2}.}
Due to Eq.~\ref{eq:GAim1_GReg2}, we want to maintain $\phi(\rmX) \to \psi(\rmY)$ but suppressing   $\psi(\rmY) \to \phi(\rmX)$. Thus we want to $ \max_{\phi,\psi} H(P(\phi(\rmX) | \psi(\rmY)), \mathcal{D})$ while $\min _{\phi,\psi}H(P( \psi(\rmY) | \phi(\rmX) ), \mathcal{D})$. which problem can be simplified as:
\begin{equation}
    \begin{split}
     % &\max_{\phi,\psi} H(P(\phi(\rmX) | \psi(\rmY)), \mathcal{D}) + \min _{\phi,\psi}H(P( \psi(\rmY) | \phi(\rmX) ), \mathcal{D}) \\ 
     &\min_{\phi,\psi} H(P( \psi(\rmY) | \phi(\rmX) , \mathcal{D} ))-H(P(\phi(\rmX) | \psi(\rmY) , \mathcal{D})) \\
     =& \min_{\phi,\psi} H(\phi(\rmX),\psi(\rmY)|\mathcal{D})) -  I(\phi(\rmX),\psi(\rmY)|\mathcal{D})) - \\
     & H(P(\phi(\rmX) | \psi(\rmY) , \mathcal{D})) + H(P(\phi(\rmX) | \psi(\rmY) , \mathcal{D})) \\
      =& \min_{\phi,\psi} H(\phi(\rmX),\psi(\rmY)|\mathcal{D})) -  I(\phi(\rmX),\psi(\rmY)|\mathcal{D})),
    \end{split}
\end{equation}
where the first term is already in \textbf{GAim2}, thus \textbf{GReg2} should deal with the second term, which is:
\begin{equation}
    \begin{split}
     &\min_{\phi,\psi} I(\phi(\rmX),\psi(\rmY)|\mathcal{D})) = \\ & \min_{\phi,\psi} H (P(\phi(\rmX))|\mathcal{D}) - H(P(\phi(\rmX))|P(\psi(\rmY)),\mathcal{D}).
    \end{split}
\end{equation}
Also, due to the effect of $\mathcal{D}$ being alleviated through the mappings, the above equation is approximated as  
\begin{equation}
    \begin{split} 
    \min_{\phi,\psi} H (P(\phi(\rmX))) - H(P(\phi(\rmX))|P(\psi(\rmY))),
    \end{split}
\end{equation}
where is \textbf{GReg2}.
% Due to $ I(\phi(\rmX),\psi(\rmY)|\mathcal{D})) $



% \begin{equation}
%     \begin{split}
%      &\max_{\phi,\psi} H(P(\phi(\rmX) | \psi(\rmY))) \\ 
%      =&\min_{\phi,\psi} -H(P(\phi(\rmX) | \psi(\rmY))) \\
%      =& \min_{\phi,\psi} - H(P(\phi(\rmX)))
%     \end{split}
% \end{equation}

% \begin{align}
%     &\quad H( P ({\phi(\rmX), \psi(\rmY)} \mid \mathcal{D}))
%     \nonumber \\ 
%     & =   H( P ({\psi(\rmY)} \mid \mathcal{D}))  + H( P ({\phi(\rmX) \mid \psi(\rmY)}, \mathcal{D}))    \nonumber \\
%     & \leq  H( P ({\psi(\rmY)} \mid \mathcal{D}))  + H( P ({ \phi(\rmX)} \mid \mathcal{D})) \nonumber \\
%     & =  H( P ({\psi(\rmY)} \mid \mathcal{D}))   \nonumber \\ 
%     & \quad \underbrace{+ H( P ({\phi(\rmX) \mid \psi(\rmY)}, \mathcal{D})) -  H( P ({\phi(\rmX) \mid \psi(\rmY)}, \mathcal{D}))}_{=0} \nonumber \\ 
%     & \quad + H( P ({ \phi(\rmX)} \mid \mathcal{D}))  \nonumber 
%     \\
%     & = \text{\textbf{GAim1}}\! - \!H( P ({\phi(\rmX) \mid \psi(\rmY)}, \mathcal{D})) + H( P ({ \phi(\rmX)} \mid \mathcal{D})).  \nonumber 
% \end{align}
% It can be reformed as:
% \begin{align}
%      &  \text{\textbf{GAim1}} - H( P ({\phi(\rmX) \mid \psi(\rmY)}, \mathcal{D})) + H(P(\psi(\rmY), \mathcal{D}))\! 
%      \nonumber 
%     \\& \quad + H( P ({ \phi(\rmX)} \mid \mathcal{D}))  \underbrace{ - H(P(\mathcal{D}))  + H(P(\mathcal{D})) }_{=0} 
%       \nonumber 
%     \\
%     =   &\text{\textbf{GAim1}}\! -\! H( P ({\phi(\rmX) \mid \psi(\rmY)}, \mathcal{D})) \!-\! H(P(\mathcal{D})) \! \nonumber 
%     \\&  + \!H(P(\psi(\rmY), \mathcal{D}))\! + \!H( P ({ \phi(\rmX)} \mid \mathcal{D}))\! +\! H(P(\mathcal{D}))  
%       \nonumber 
%     \\
%     =  & \text{\textbf{GAim1}}  -  H( P ({\phi(\rmX) \mid \psi(\rmY)}))   + \! H( P ({ \phi(\rmX)}) \nonumber 
%     \\
%    =  & \text{\textbf{GAim1}}  +  \text{\textbf{GReg2}}. \nonumber  
% \end{align}

\textbf{Derivation details of Eq.~\ref{eq:cfs_detial}.}
For a Gaussian distribution $\mathcal{N}(x; \mu, \Sigma)$ with $D$ dimension, its entropy is:
% \begin{align}
%     H(x) = & - \int p(x) \ln{p(x)} dx 
%     \\ 
%     = & - \int p(x) [\ln{((2\pi)^{-\frac{D}{2}}|\Sigma|^{-\frac{1}{2}})} 
%     \nonumber 
%     \\&  - \frac{1}{2}(x-\mu)^\top \Sigma^{-1} (x-\mu) ] dx
%     \nonumber \\ 
%     = & \ln{((2\pi)^{\frac{D}{2}}|\Sigma|^{-\frac{1}{2}}) } \nonumber 
%     \\&  + \frac{1}{2} \int p(x)[(x-\mu)^\top \Sigma^{-1} (x-\mu)] dx
%     \nonumber \\ 
%     = & \ln{((2\pi)^{\frac{D}{2}}|\Sigma|^{-\frac{1}{2}}) } + \frac{1}{2} \int p(y) \times y^{\top} dy
%     \nonumber \\ 
%      = & \ln{((2\pi)^{\frac{D}{2}}|\Sigma|^{-\frac{1}{2}}) } + \frac{1}{2} \sum_{d=1}^D \mathbb{E}[y_d^2]
%     \nonumber \\ 
%      = & \ln{((2\pi)^{\frac{D}{2}}|\Sigma|^{-\frac{1}{2}}) } + \frac{D}{2}
%       \\
%     = & \frac{D}{2}(1 + \ln{(2\pi) }) + \frac{1}{2} \ln{|\Sigma|}.
%     \nonumber
% \end{align}
\begin{equation}
    \begin{split}
        H(x) = & - \int p(x) \ln{p(x)} dx 
    \\ 
    = & - \int p(x) [\ln{((2\pi)^{-\frac{D}{2}}|\Sigma|^{-\frac{1}{2}})}  
    \\&  - \frac{1}{2}(x-\mu)^\top \Sigma^{-1} (x-\mu) ] dx
     \\ 
    = & \ln{((2\pi)^{\frac{D}{2}}|\Sigma|^{-\frac{1}{2}}) }  
    \\&  + \frac{1}{2} \int p(x)[(x-\mu)^\top \Sigma^{-1} (x-\mu)] dx
     \\ 
    = & \ln{((2\pi)^{\frac{D}{2}}|\Sigma|^{-\frac{1}{2}}) } + \frac{1}{2} \int p(y) \times y^{\top} dy
     \\ 
     = & \ln{((2\pi)^{\frac{D}{2}}|\Sigma|^{-\frac{1}{2}}) } + \frac{1}{2} \sum_{d=1}^D \mathbb{E}[y_d^2]
     \\ 
     = & \ln{((2\pi)^{\frac{D}{2}}|\Sigma|^{-\frac{1}{2}}) } + \frac{D}{2}
      \\
    = & \frac{D}{2}(1 + \ln{(2\pi) }) + \frac{1}{2} \ln{|\Sigma|}.
    \end{split}
\end{equation}
% \textbf{Derivation details of Eq.~\ref{eq:for_pred} and  Eq.~\ref{eq:larg_mult}.}
% To learn the predictor, we need to:
% \begin{align}
%     &\max_{\phi, \psi} P(\rmY \mid \phi(\rmX)) P(\rmY \mid \psi(\rmY)) \nonumber \\
%      = &\max_{\phi, \psi} I(P(\phi(\rmX)), {P(\rmY)}) + I(P(\phi(\rmY)), P(\rmY))  \nonumber \\
%     = &   \max_{\phi, \psi} [H(P(\phi(\rmX))) + H(P(\rmY)) - H(P(\phi(\rmX), \rmY)) ]+  \nonumber
%      \\ & [H(P(\psi(\rmY))) + H(P(\rmY)) - H(P(\psi(\rmY), \rmY)) ]  \nonumber
%     \\  
%     = &  \min_{\phi, \psi}  H((P(\phi(\rmX), \rmY)) + 
%     H((P(\psi(\rmY), \rmY)) - H(P(\phi(\rmX)))
%     - H(P(\psi(\rmY)))
%     - \underbrace{2H(P(\rmY))}_{\text{constant}}  \nonumber
%      \\  
%     % = & \min_{\phi, \psi}   H((P(\phi(\rmX), \rmY)) + 
%     % H((P(\psi(\rmY), \rmY)) - H(P(\phi(\rmX)))
%     % - H(P(\psi(\rmY))) + H(P(\phi(\rmX), \psi(\rmY)) -  H(P(\phi(\rmX), \psi(\rmY)) \nonumber
%     %  \\  
%     %   = & \min_{\phi, \psi}   H((P(\phi(\rmX), \rmY)) + 
%     % H((P(\psi(\rmY), \rmY))
%     % - I (P(\phi(\rmX)), P(\psi(\rmY)))  -  H(P(\phi(\rmX), \psi(\rmY)) 
%          = & \min_{\phi, \psi}   H((P(\phi(\rmX), \rmY))  - H(P(\phi(\rmX))) + 
%     H((P(\psi(\rmY), \rmY))  - H(P(\psi(\rmY)))  \nonumber \\
%     % - I (P(\phi(\rmX)), P(\psi(\rmY)))  -  H(P(\phi(\rmX), \psi(\rmY)) \\ 
%        = & \min_{\phi, \psi}   H((P(\rmY \mid\phi(\rmX))) + 
%     H((P(\rmY \mid \psi(\rmY))).  \nonumber
% \end{align}
% Using \textit{Lagrange Multiplier}, from  Eq.~\ref{eq:for_pred} we have Eq.~\ref{eq:larg_mult}:
% \begin{align}
%      &\max_{\phi, \psi} H(P(\rmY \mid \phi(\rmX))) + H(P(\rmY \mid \psi(\rmY))) - v_{R2} I(\phi(\rmX);\psi(\rmY)) . 
% \end{align}



Then Eq.~\ref{eq:cfs_detial} equals: 
% \begin{align}
% \label{eq:cfs_detial_proof}
%     & H( \mathcal{N}(\phi(\rmX); \mu_\rmX, \Sigma_{\rmX\rmX})) \nonumber 
%     \\& - H( \mathcal{N}(\phi(\rmX)\mid \psi(\rmY); \mu_{\rmX|\rmY}, \Sigma_{\rmX\rmX|\rmY}))  
%     \\
%     =&\frac{D}{2} (1 + \ln(2\pi)) + \frac{1}{2} \ln| \Sigma_{\rmX\rmX} | \nonumber 
%     \\&  -  \frac{D}{2} (1 + \ln(2\pi)) - \frac{1}{2} \ln| \Sigma_{\rmX\rmX|\rmY} |  
%      \\
%      = & \frac{1}{2} \ln(|\Sigma_{\rmX\rmX}|) - \ln(|\Sigma_{\rmX\rmX|\rmY}|), \nonumber
%     \\
%      = & \frac{1}{2} \ln(\frac{|\Sigma_{\rmX\rmX}|}{|\Sigma_{\rmX\rmX|\rmY}|}). \nonumber
% \end{align}
\begin{equation}
\label{eq:cfs_detial_proof}
    \begin{split}
        & H( \mathcal{N}(\phi(\rmX); \mu_\rmX, \Sigma_{\rmX\rmX}))  
    \\& - H( \mathcal{N}(\phi(\rmX)\mid \psi(\rmY); \mu_{\rmX|\rmY}, \Sigma_{\rmX\rmX|\rmY}))  
    \\
    =&\frac{D}{2} (1 + \ln(2\pi)) + \frac{1}{2} \ln| \Sigma_{\rmX\rmX} |  
    \\&  -  \frac{D}{2} (1 + \ln(2\pi)) - \frac{1}{2} \ln| \Sigma_{\rmX\rmX|\rmY} |  
     \\
     = & \frac{1}{2} \ln(|\Sigma_{\rmX\rmX}|) - \ln(|\Sigma_{\rmX\rmX|\rmY}|), 
    \\
     = & \frac{1}{2} \ln(\frac{|\Sigma_{\rmX\rmX}|}{|\Sigma_{\rmX\rmX|\rmY}|}). 
    \end{split}
\end{equation}

\textbf{Empirical risk.}
The empirical risk introduced by the whole model $\theta$ \textit{w.r.t} $\rmX, \rmY$ is determined by a convex loss function $L(\theta)$. Following ~\citep{perlaza2022empirical},
the empirical risk considering $\mathcal{O}$ is:
 \begin{align}
 % \label{eq:erm}
     R(\theta) = & \int L(\theta)dP(\theta) +  H(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})]) \nonumber 
    \\&  + \KL( \mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})] \Vert \; \mathcal{O}) \\ & - H(P(\phi(\rmX)  \mid  \psi(\rmY))) 
        + H(P(\phi(\rmX))) . \nonumber
\end{align}


\textbf{Proof of \textbf{Using $\psi$ \textit{v.s.} not using $\psi$}.} 
% \begin{lemma} 
% \label{le:equal} 
Using \textit{ Jensen’s inequality}, due to $\rmY, \psi(\rmY)$ contains the same amount of useful information as $\rmY$, we have:
\begin{align}
    H(\rmY) \ge H(\psi(\rmY)).
\end{align}


Therefore, we have
% \begin{align}
%      &H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})]) \\
%      =  &H(\mathbb{E}[ P (\phi(\rmX_n))]) + H(\mathbb{E}[ P ({\rmY_n \mid \phi(\rmX_n) })]) \nonumber \\
%      \ge & H(\mathbb{E}[ P (\phi(\rmX_n))]) + H(\mathbb{E}[ P ({\psi(\rmY_n )\mid \phi(\rmX_n) })])  \nonumber \\
%      = &H(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})]) . \nonumber 
% \end{align}
\begin{equation}
    \begin{split}
    &H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})]) \\
     =  &H(\mathbb{E}[ P (\phi(\rmX_n))]) + H(\mathbb{E}[ P ({\rmY_n \mid \phi(\rmX_n) })])  \\
     \ge & H(\mathbb{E}[ P (\phi(\rmX_n))]) + H(\mathbb{E}[ P ({\psi(\rmY_n )\mid \phi(\rmX_n) })])   \\
     = &H(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})]) .  
    \end{split}
\end{equation}
Therefore, for the risk of $\theta^{n\psi}$:
 \begin{align}
     \sup R({\theta}^{n\psi}) =  \sup & \min_{\phi} [\int L(\theta)dP(\theta) \nonumber 
    \\& +  H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})])] + b,
 \end{align}
and the risk of $\theta^{n\psi}$:
\begin{align}
     \sup R({\theta}^{\psi}) =  \sup & \min_{\phi} [\int L(\theta)dP(\theta) \nonumber 
    \\& +  H(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})])] + b,
 \end{align}
 where $b \triangleq \KL( \mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})] \Vert \; \mathcal{O})   - H(P(\phi(\rmX)  \mid  \psi(\rmY))) + H(P(\phi(\rmX))) , $  we have:
 \begin{align}
     \sup R({\theta}^{n\psi}) \ge \sup R({\theta}^{\psi}) .
 \end{align}
%  For $R(\hat{\theta})$, it has:
% % If the assumption that $\psi$ is a one-to-one mapping holds, 
% % We have the following:
% %     $PUB(P ({\phi(\rmX),\psi(\rmY) \mid \mathcal{D}})) 
% %     \ge PUB(P ({\phi(\rmX),\rmY \mid \mathcal{D}}))$ .
% % \end{lemma}
% % Lemma~\ref{le:equal} can be easily proofed by using \textit{Jensen's inequality}. 
% % \begin{proof}
% Based on \textit{Jensen's inequality}, we have $H(\psi(\rmY)) \ge H(\rmY)$, thus:
% \begin{align}
%  & \min_{\phi, \psi}{ H(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})])} + {\KL(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)}) ] \Vert\mathcal{O}))}  -{a} \nonumber 
%  \\ 
% % \leq \min_{Q\in\mathcal{Q}} H_c(P_{mix}, Q) -  \mathbb{E}[ H (P_{\phi(X_i), \psi(Y_i)})],
% \ge & \min_{\phi, \psi}{ H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})])} + {\KL(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n}) ] \Vert\mathcal{O}))}  -a \nonumber 
% \end{align}
% thus Lemma~\ref{le:equal} holds and the equivalence only can be achieved when $\phi$ is a one-to-one mapping. 
% \end{proof}


\textbf{Proof of incorporating conditions leads to lower generalization risk on learning invariant representations.}
For the risks of the model having parameters $\theta^{c}$ trained with using conditions, we have:
 \begin{align}
     \sup R({\theta}^{c}) =  \sup & \min_{\phi} [\int L(\theta)dP(\theta) \nonumber 
    \\& +  H(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})])] + b,
 \end{align}
 where $b \triangleq \KL( \mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})] \Vert \; \mathcal{O})   - H(P(\phi(\rmX)  \mid  \psi(\rmY))) + H(P(\phi(\rmX))) . \nonumber$ For $R({\theta}^{nc})$ that trained without using conditions, it has:
  \begin{align}
     \sup R({\theta}^{nc}) = \sup & \min_{\phi,\psi} [ \; \int L(\theta)dP(\theta)  +  H(\mathbb{E}[ P ({\phi(\rmX_n)})])  \;  ] \nonumber 
    \\&  + H(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})])  \nonumber \\ 
     & -  H(\mathbb{E}[ P ({\phi(\rmX_n)})]) + b   \\
      = \sup & \min_{\phi,\psi} [\;\int L(\theta)dP(\theta)  +  H(\mathbb{E}[ P ({\phi(\rmX_n)})]) \;] \nonumber 
    \\& + H(\mathbb{E}[ P ({ \psi(\rmY_n) \mid \phi(\rmX_n)})]) +b. \nonumber 
 \end{align}
Due to the inequality:
\begin{align}
    &\sup  \min_{\phi} [ \; H(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})]) \;] 
    \\ = &\sup  \min_{\phi} [ \; H(\mathbb{E}[ P ({\phi(\rmX_n)})]) \nonumber 
    \\&  + H(\mathbb{E}[ P ({ \psi(\rmY_n) \mid \phi(\rmX_n)})]) \;] 
    \\\leq & \sup  \min_{\phi,\psi} [ \;H(\mathbb{E}[ P ({\phi(\rmX_n)})]) \;] \nonumber 
    \\& + H(\mathbb{E}[ P ({ \psi(\rmY_n) \mid \phi(\rmX_n)})]),
\end{align}
we have
\begin{align}
     \sup R({\theta}^{nc}) \ge \sup R({\theta}^{c}) .
\end{align}


% \textbf{Proof of using $\mathcal{O}$ that only trained on seen domains.}
% A special case is $\mathcal{O}$ trained solely on seen domains, i.e., $\mathcal{O}\triangleq P^* (\phi(\rmX), \psi(\rmY)) $. In this case, the PUB is altered as:
% \begin{align}
% \label{eq:orcale_bound2}
%     &\min\nolimits_{\phi,\psi} H(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})]) + \underbrace{\KL( P (\phi(\rmX), \psi(\rmY)) \Vert P^* (\phi(\rmX), \psi(\rmY)))}_{\text{Diminished with } \mathcal{L}_{pred},  \text{ omitted.}}-a .
%     % \\
%     % =  &\min_{\phi} H(\mathbb{E}[ P ({\phi(\rmX_n), \psi(\rmY_n)})])
% \end{align}


\section{Objective derivation details of many previous methods.}
\label{app:pre_obj}

This section shows how we uniformly simplify the objectives of previous methods. 
% In this section, we discuss how current typical domain generalization methods learn the $\mathcal{D}$-independent conditional features. 
% Specifically, we uniformly simplify their objectives on and link them to our DUAUB. 
% and compare them to ours regarding \textbf{Aim~1} and \textbf{Aim~2}. 
% Thus the equation holds.
% \end{proof}

% There are multiple attempts to obtain invariant features.

% Table~\ref{tab:summary} summarizes the objectives of related current methods and ours, and corresponding mathematical derivation details are shown. 
% We developed the previous related works. Then we compare them with our PUB.
% compare our PUB. with other upper bounds on GJSD of previous related works.
% \subsection{Previous objectives for \textbf{Aim~1}}'



\textbf{ERM~\citep{gulrajani2020search}: The basic method.} 
The basic method does not focus on minimizing GJSD. Therefore, there are no terms for \textbf{Aim~1}. For \textbf{Aim~2} it directly minimize $H(P ({\phi(\rmX), \rmY}))$.
% it only focuses the $\max_{\phi}P ({ \phi(X) \mid Y})$ without minimizing .


\textbf{DANN~\citep{ganin2016domain}: Minimize feature divergences of source domains.} DANN~\citep{ganin2016domain} minimizes feature divergences of source domains adverbially without considering conditions. Therefore its empirical objective for \textbf{Aim~1} is 
\begin{align}
    &\min_{\phi} H(\mathbb{E}[ P ({\phi(\rmX_n)})]) -a
    % =  & \min_{\phi} H( P ({\phi(\rmX)} \mid \mathcal{D})]) 
\end{align}
For \textbf{Aim~2} it directly minimizes $H(P ({\phi(\rmX), \rmY}))$.

\textbf{CORAL~\cite{sun2016deep}: Minimize the distance between the second-order statistics of source domains.} Since CORAL~\cite{sun2016deep} only minimizes the second-order distance between souce feature distributions, its objective
can be summarized as:
% for \textbf{Aim~1} is as:
\begin{align}
    % = \mathbb{E}[\KL(P(\phi(\rmX_n)) \Vert \mathbb{E}[P(\phi(\rmX_n))] ) - \KL( P(\mathbb{E}[\phi(\rmX_n)]) \Vert \mathbb{E}[P(\phi(\rmX_n))] ) ] \\
    % = min_{\phi} H(\mathbb{E}[ P ({\phi(\rmX_n)})]) - \underbrace{\KL( \mathbb{E}[P(\mathbb{E}[\phi(\rmX_n)])] \Vert \mathbb{E}[P(\phi(\rmX_n))] )}_{\ge 0}.
   \min_{\phi} 
   % H(P ({\phi(\rmX), \rmY})) - H(\mathbb{E}[P({\phi(\rmX_n)})]) + {H(P({\phi(\rmX)}))}.
    H(P ({ \phi(\rmX) , \rmY}))+ H(P({\phi(\rmX)})) -H(\mathbb{E}[ P ({\phi(\rmX_n)})]) .
\end{align}
% For \textbf{Aim~2} it directly minimizes $H(P ({\phi(\rmX), \rmY}))$.
By grouping it, CORAL~\citep{sun2016deep} has $ -H(\mathbb{E}[ P ({\phi(\rmX_n)})])$ for \textbf{Aim~1} and $H(P ({ \phi(\rmX) , \rmY}))+ H(P({\phi(\rmX)}))$ for \textbf{Aim~2}. 


\textbf{CIDG~\citep{li2018domain}: Minimizing the conditioned domain gap.} CIDG~\citep{li2018domain} tries to learn conditional domain invariant features:  
\begin{align}
\label{eq:CIDG} 
    \min_{\phi} H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})]).
\end{align}
For \textbf{Aim~2} it directly minimizes $H(P ({\phi(\rmX), \rmY}))$.



\textbf{MDA~\citep{hu2020domain}: Minimizing domain gap compared to the decision gap.} 
% Some previous works~\cite{muandet2013domain, li2018domain} follow the hypnosis that the generalization is guaranteed while the decision gap is larger than the domain gap. Therefore, instead of directly minimizing the domain gap, \cite{muandet2013domain} minimize the ratio between the domain gap and the decision gap which can be summarized as:
Some previous works, such as MDA~\citep{hu2020domain}, follow the hypothesis that the generalization is guaranteed while the decision gap is larger than the domain gap. Therefore, instead of directly minimizing the domain gap, MDA minimizes the ratio between the domain gap and the decision gap. The overall objective of MDA can be summarized as:
% \begin{align}
% \label{eq:MDA}
%     % &\min_{\phi,\psi} \frac{ \mathbb{E}[KL(P_{\phi(X_{n}), \psi(Y_n)}, \mathbb{E}[P_{\phi(X_{n}), \psi(Y_n)}])]} {\mathbb{E}[ KL(P_{\phi(X_n)}, \mathbb{E}[P_{\phi(X_{n})}])]} \nonumber \\
%     % =  &\min_{\phi,\psi} \frac{H(\mathbb{E}[ P_{\phi(X_n), \psi(Y_n)}]) - \mathbb{E}[H (P_{\phi(X_n),\psi(Y_n)})]}
%     % {H(\mathbb{E}[ P_{\phi(X_n)}]) - \mathbb{E}[H (P_{\phi(X_n)})]},
%     % &\min_{\phi} \frac{ \mathbb{E}[\KL(P ({\phi(\rmX_{n}) , \rmY_n}) \Vert \mathbb{E}[P ({\phi(\rmX_{n}), \rmY_n})])]} {\mathbb{E}[ \KL(P ({\phi(\rmX_n) \mid \rmY_n}) \Vert \mathbb{E}[P ({\phi(\rmX) \mid \rmY})])]} + {\mathbb{E}[H(P ({\phi(\rmX), \rmY}))]} + H(P ({\phi(\rmX), \rmY})) + H(P (\phi(\rmX)))\\
%     &\min_{\phi}  H(P ({\phi(\rmX), \rmY})) + H(P (\phi(\rmX)))  
%     \\& +  ({H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})]) - \underbrace{\mathbb{E}[H (P ({\phi(\rmX_n),\rmY_n}))]}_{constant}}) \nonumber \\
%     & - ({H(\mathbb{E}[ P({\phi(\rmX_n)\mid \rmY_n})]) - \underbrace{ \mathbb{E}[H (P ({\phi(\rmX)\mid \rmY}))]}_{constant}}) \nonumber 
%     \\& + \underbrace{\mathbb{E}[H(P ({\phi(\rmX), \rmY}))]}_{constant} \nonumber.
% \end{align}
\begin{equation}
    \begin{split}
    \label{eq:MDA}
    &\min_{\phi}  H(P ({\phi(\rmX), \rmY})) + H(P (\phi(\rmX)))  
    \\& +  ({H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})]) - \underbrace{\mathbb{E}[H (P ({\phi(\rmX_n),\rmY_n}))]}_{constant}})  \\
    & - ({H(\mathbb{E}[ P({\phi(\rmX_n)\mid \rmY_n})]) - \underbrace{ \mathbb{E}[H (P ({\phi(\rmX)\mid \rmY}))]}_{constant}})  
    \\& + \underbrace{\mathbb{E}[H(P ({\phi(\rmX), \rmY}))]}_{constant} .
    \end{split}
\end{equation}
% where $\mathbb{E}[H (P_{\phi(X_n),\psi(Y_n)})]$, $\mathbb{E}[H (P_{\phi(X_n)})]$ are constants and can be omitted during optimization. Eq.~(\ref{eq:invaraint_bound_pre}) is equivalent to:
% where $\mathbb{E}[H (P ({\phi(\rmX_n),\rmY_n}))]$, $\mathbb{E}[H (P ({\phi(\rmX_n)\mid \rmY_n}))]$ are constants and can be omitted during optimization.
% Note that DICA assumes $P(\rmY)$ is stable while $P(\rmX|\rmY)$ changes across domains. 


% \begin{proposition}
%     Using Eq.~\ref{eq:invaraint_bound_pre} as an optimization objective leads to sub-optimal results.
% \end{proposition}

% \begin{proof}
    Since  the entropy is non-negative and the constants can be omitted, Eq.~\ref{eq:MDA} is equivalent to:
% \begin{align}
% \label{eq:MDA2}
%     % min_{\phi,\psi} & H(\mathbb{E}[ P ({\phi(X_n), Y_n})])-  H(\mathbb{E}[ P ({\phi(X_n)\mid Y_n})])).  
%     &\min_{\phi} H(P ({\phi(\rmX), \rmY})) + H(P (\phi(\rmX))) 
%     \\
%     & + H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})])-  H(\mathbb{E}[ P({\phi(\rmX)\mid \rmY})])) + a. \nonumber 
%     % \\ \nonumber
%     %  =&\min_{\phi} H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})])-  H(\mathbb{E}[ \frac{P({\phi(\rmX_n)}) P(\rmY_n \mid \phi(\rmX_n))}{ P(\rmY_n)}])) \\ \nonumber
%     %  =&\min_{\phi} H(\mathbb{E}[ P ({\phi(X_n), Y_n})])- 
%     % H(\mathbb{E}[ P({\phi(\rmX_n)}) \underbrace{P(\rmY_n \mid \phi(\rmX_n))}_{\text{Bounded by} \mathcal{L}_{pred}, \text{omitted.}}])) 
%     %  \\
%     %   \triangleq &
%     %  \min_{\phi} H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})])-  H(\mathbb{E}[ P({\phi(\rmX_n)})]))
%     % \nonumber 
%     % \\
%     % &  - \mathbb{E}[H (P ({\phi(X_n),Y_n})]  + \mathbb{E}[H (P ({\phi(X_n)}))].
% \end{align}
% \begin{align}
% \label{eq:MDA2}
%     % min_{\phi,\psi} & H(\mathbb{E}[ P ({\phi(X_n), Y_n})])-  H(\mathbb{E}[ P ({\phi(X_n)\mid Y_n})])).  
%     &\min_{\phi} H(P ({\phi(\rmX)\mid \rmY})) + H(P (\phi(\rmX))) 
%     \\
%     & + H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})])-  H(\mathbb{E}[ P({\phi(\rmX)\mid \rmY})])) + a. \nonumber 
%     % \\ \nonumber
%     %  =&\min_{\phi} H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})])-  H(\mathbb{E}[ \frac{P({\phi(\rmX_n)}) P(\rmY_n \mid \phi(\rmX_n))}{ P(\rmY_n)}])) \\ \nonumber
%     %  =&\min_{\phi} H(\mathbb{E}[ P ({\phi(X_n), Y_n})])- 
%     % H(\mathbb{E}[ P({\phi(\rmX_n)}) \underbrace{P(\rmY_n \mid \phi(\rmX_n))}_{\text{Bounded by} \mathcal{L}_{pred}, \text{omitted.}}])) 
%     %  \\
%     %   \triangleq &
%     %  \min_{\phi} H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})])-  H(\mathbb{E}[ P({\phi(\rmX_n)})]))
%     % \nonumber 
%     % \\
%     % &  - \mathbb{E}[H (P ({\phi(X_n),Y_n})]  + \mathbb{E}[H (P ({\phi(X_n)}))].
% \end{align}
\begin{equation}
    \begin{split}
    \label{eq:MDA2}
    &\min_{\phi} H(P ({\phi(\rmX)\mid \rmY})) + H(P (\phi(\rmX))) 
    \\
    & + H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})])-  H(\mathbb{E}[ P({\phi(\rmX)\mid \rmY})])) + a.  
    \end{split}
\end{equation}
By grouping Eq.~\ref{eq:MDA2}, we have that for \textbf{Aim~1} it minimizes $\min_{\phi} H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})])$, and for \textbf{Aim~2} it minimizes $H(P ({\phi(\rmX)\mid\rmY})) -  H(\mathbb{E}[ P({\phi(\rmX) \mid \rmY})])) +  H(P (\phi(\rmX)))$. 



% Due to Lemma~\ref{le:equal}, the first term in Eq.~\ref{eq:invaraint_bound} is the same as (1)~term in PUB, suggesting that only (1)~term in PUB is minimized. Furthermore, even adding $\KL(P_{mix} \Vert\mathcal{O}))$ to Eq.~\ref{eq:invaraint_bound}, 
% the minimization is hindered by $H(\mathbb{E}[ P({\phi(\rmX_n)})]$ as it is non-negative. Therefore, Eq.~\ref{eq:invaraint_bound} leads to sub-optimal results.
% \end{proof}
 


% Similarly, \cite{li2018domain}'s GJSD upper bound is Eq.~(\ref{eq:invaraint_bound}) without $\psi$. Note that \cite{muandet2013domain} is a machine learning without employing deep neural networks.

% \begin{proposition} PUB provides a tighter upper bound than Eq.~(\ref{eq:invaraint_bound}). 
% % if $ O ({X, Y})$ is only about seen $X,Y$.
% \end{proposition}
% \begin{proof}
%     With constants omitted,  Eq.~(\ref{eq:invaraint_bound}) is reformed as:
%     \begin{align}
%         min_{\phi,\psi} H(\mathbb{E}[ P ({\phi(X_n), Y_n})])-  H(\mathbb{E}[ P ({\phi(X_n)\mid Y_n})])),
%     \end{align}
%     where based on Lemma.~\ref{le:equal} Eq.~(\ref{eq:PUB}) is as:
%     \begin{align}
%         \min_{\phi, \psi} H(\mathbb{E}[ P_{\phi(X_n), Y_n}]) + KL(P_{mix},  O ({X, Y}) ).
%     \end{align}
%     Due to KL and entropy's non-negativity, Eq.~(\ref{eq:PUB}) provides a tighter bound than Eq.~(\ref{eq:invaraint_bound}), even without considering $KL(P_{mix},  O ({X, Y}) )$.
% \end{proof}

% It also suggests that Eq.~(\ref{eq:invaraint_bound}) cannot guarantee a generalization.
% \subsubsection{\red{Training $O ({X, Y})$ on $X,Y$.}} 
% It is feasible to  

% \subsubsection{Obtaining $O ({X, Y})$ on $X,Y$}



\textbf{MIRO~\citep{cha2022miro}, SIMPLE~\citep{li2022simple}: Using pre-trained models as $ \mathcal{O}$.} 
One feasible way to obtain $\mathcal{O}$ is adopting pre-trained oracle models such as MIRO~\citep{cha2022miro} and SIMPLE~\citep{li2022simple}. Note that the pre-trained models are exposed to additional data besides those provided. Therefore, for \textbf{Aim~1}: they have: 
% Specifically, the adopted pre-train models capture $\mathcal{O}$ which is used to constrain $P(\phi(\rmX))$.
% We provide the objective of minimizing GJSD of current methods that use pre-trained models as $ \mathcal{O}$, such as MIRO~\cite{cha2022miro} and SIMPLE~\cite{li2022simple} :
\begin{align}
\label{eq:orcale_bound}
    \min_{\phi} \KL( P (\phi(X)|Y) \Vert\mathcal{O})-  \underbrace{\mathbb{E}[ H (P ({\phi(\rmX_n),\rmY_n}))]}_{constant}.
\end{align}
% Due to $O(\rmY)$ have been assumed stable across domains, Eq.~\ref{eq:orcale_bound} is equivalent:
% \begin{align}
%     &\min_{\phi} KL(  P_{mix},  O ({\rmX|\rmY})O(\rmY))-  \mathbb{E}[ H (P ({\phi(\rmX_n),\rmY_n}))]. \nonumber
%     \\
%     =&\min_{\phi} KL( P_{mix}, \mathcal{O})-\mathbb{E}[ H (P({\phi(\rmX_n),\rmY_n}))].
% \end{align}
Differently, MIRO only uses one pre-trained model, as its $\mathcal{O} \triangleq  \mathcal{O}^1$; meanwhile, SIMPLE combines $K$ pre-trained models as the oracle model: $\mathcal{O} \triangleq \sum_{k=1}^{K} v_k  \mathcal{O}^k$ where $v$ is the weight vector.  
% \begin{proposition}
%     Using Eq.~\ref{eq:orcale_bound} as an optimization objective leads to sub-optimal results.
% \end{proposition}
% \begin{proof}
    % With Lemma~\ref{le:equal}, the first term in Eq.~\ref{eq:orcale_bound} is the (2)~term in PUB. Thus using
    % Eq.~\ref{eq:orcale_bound} as the objective only minimizes a partial of PUB, triggering sub-optimal results.
% \end{proof}
For \textbf{Aim~2} it directly minimizes $H(P ({\phi(\rmX), \rmY}))$.



\textbf{RobustNet~\citep{choi2021robustnet}.} RobustNet employs the instance selective whitening loss, which disentangles domain-specific and domain-invariant properties from higher-order statistics of the feature representation and selectively suppresses domain-specific ones. Therefore, it implicitly whitens the $\rmY$-irrelevant features in $\rmX$. Thus, its objective can be simplified as:
% \begin{align}
%      &\min_{\phi,{\psi}}H(P ({ \phi(\rmX) , {\psi(\rmY)}}))  - H(P(\phi(\rmX)  \mid  \psi(\rmY))) 
%       \nonumber 
%     \\&   + H(P(\phi(\rmX))).
% \end{align}
% By omitting $2$, its objective can be rewritten as:
\begin{equation}
    \begin{split}
         &\min_{\phi,{\psi}}H(P ({ \phi(\rmX) , {\psi(\rmY)}}))  - H(P(\phi(\rmX)  \mid  \psi(\rmY))) 
    \\&   + H(P(\phi(\rmX))).
    \end{split}
\end{equation}


\section{Aligning notations between paper and supplementary materials}
\subsection{More details about Table~\ref{tab:summary}}
To better understand, we simplify some notations in Table~\ref{tab:summary}. We present the simplified notations and their corresponding origins in Table~\ref{tab:summary2}.

\begin{table*}[t]
\begin{center}
% \scriptsize
% \resizebox{\linewidth}{!}{%
\begin{tabular}{lll}
\toprule
 & \multicolumn{2}{c}{ \bf Learning domain invariant representations}\\ 
 & \multicolumn{1}{c}{\bf Aim1: Learning domain invariance} & \multicolumn{1}{c}{\bf Reg1: Integrating prior} \\ \midrule
% ERM,CORAL,RobustNet & None & None \\ 
\specialrule{0em}{3pt}{3pt}
DANN & $\min_{\phi} H(  P (\phi(\rmX) \mid \mathcal{D}))$ & None \\
  & \blue{$\min_{\phi} H( \mathbb{E}[ P (\phi(\rmX_{n})) ]$} &  \\ \specialrule{0em}{3pt}{3pt}
CDANN, CIDG, MDA & $\min_{\phi} H(  P ({\phi(\rmX), \rmY} \mid \mathcal{D}))$ & None \\
  & \blue{$\min_{\phi} H( \mathbb{E}[ P (\phi(\rmX_{n}), \psi( \rmY_n)) ]$} &  \\ \specialrule{0em}{3pt}{3pt}
% MIRO, SIMPLE & None & $\min_{\phi} \KL(P({\phi(\rmX), \rmY})\Vert \mathcal{O})$ \\ \hline
\textbf{Ours} & {$\min_{\phi, \psi} H( P ({\phi(\rmX), \psi(\rmY)} \mid \mathcal{D}))$} & {${\min_{\phi, \psi}\KL(P({\phi(\rmX), \psi(\rmY)})\Vert \mathcal{O})}$} \\
 & \blue{$\min_{\phi, \psi} H(  \mathbb{E}[P ({\phi(\rmX_N), \psi(\rmY_n)}])$} \\ \specialrule{0em}{3pt}{3pt}
\bottomrule \toprule
 & \multicolumn{2}{c}{ \bf Maximizing A Posterior between representations and targets}\\ 
 & \multicolumn{1}{c}{ \bf Aim2: Maximizing A Posterior (MAP)}   & \multicolumn{1}{c}{ \bf Reg2: Suppressing invalid causality}\\ \midrule \specialrule{0em}{3pt}{3pt}
% Others &{$\min_{\phi}H(P ({\rmY \mid  \phi(\rmX)}))$} & None \\ \hline
CORAL & {$\min_{\phi}H(P ({\rmY \mid  \phi(\rmX)}))$} & {$\min_{\phi}-H( P ({\phi(\rmX\mid \mathcal{D} )})) + H(P({\phi(\rmX)}))$} \\ 
  &   & \blue{$\min_{\phi}-H( \mathbb{E}[P ({\phi(\rmX_n)})]) + H(P({\phi(\rmX)}))$} \\ 
  \specialrule{0em}{3pt}{3pt}
  % \hline 
% MDA,RobutsNet & {$\min_{\phi}H(P ({\rmY \mid  \phi(\rmX)}))$} & {$\min_{\phi} -  H ( P({\phi(\rmX)\mid \rmY}))  +  H(P (\phi(\rmX))) $} \\ 
% \textbf{Ours} &\blue{$\min_{\phi,\psi}H(P ({\psi(\rmY) \mid  \phi(\rmX)})) + H(P ({\rmY \mid  \psi(\rmY)}))$} & \blue{${\min_{\phi} - H(P(\phi(\rmX)  \mid  \psi(\rmY))) +H(P(\phi(\rmX)))}$}  \\
\bottomrule
\end{tabular}%
% }
\caption{Supplemental notations for Table~\ref{tab:summary}. Refined notations and their original formulations are reported. The original formulations are highlighted as \blue{blue}. }
\label{tab:summary2}
\end{center}
\end{table*}
% DANN~\citep{ganin2016domain},
% CORAL~\citep{sun2016deep},
% CDANN~\cite{li2018deep}, 
% CIDG~\citep{li2018domain}, MDA~\citep{hu2020domain}, MIRO~\citep{cha2022miro}, SIMPLE~\citep{li2022simple},
% RobustNet~\citep{choi2021robustnet},
% VA-DepthNet~\cite{liu2023va}
% and our approach. 

\subsection{More details about Table~\ref{tab:note}}
For simplification, we uniformly simplified the formulation of terms from their derivation. The simplified form in Table~\ref{tab:note} and its original form can be seen in  Table~\ref{tab:note_align}. Note that the \textbf{iAim1} is from CDANN~\cite{li2018deep}, CIDG~\citep{li2018domain}, MDA~\citep{hu2020domain} and \textbf{iReg2} is from CORAL~\citep{sun2016deep}.


\begin{table}[t]
    \centering
    % \begin{center}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{llll}
% \multicolumn{4}{c}{\bf Notations for terms} \\ 
\toprule
\textbf{GAim2} & $H(P ({\psi(\rmY) \mid  \phi(\rmX)})) + H(P ({\rmY \mid  \psi(\rmY)}))$ &  \\ 
\textbf{GReg1} & $\KL(P ({\phi(\rmX), \rmY} \mid \mathcal{D}) \Vert \mathcal{O}))$  \\ 
\textbf{iAim1} & $H( P ({\phi(\rmX)} \mid \mathcal{D}))$ & \\ 
\textbf{GAim1} & $ H(  P ({\phi(\rmX), \rmY}) \mid \mathcal{D})$  \\
\textbf{iReg2} & $ -H( P ({\phi(\rmX)} , \mathcal{D}) + H(P({\phi(\rmX)}))$ & \\ 
\textbf{GReg2} & ${ - H(P(\phi(\rmX)  \mid  \psi(\rmY))) 
+ H(P(\phi(\rmX)))}$ \\  
\bottomrule
\toprule
\textbf{GAim2} & $H(P ({\psi(\rmY) \mid  \phi(\rmX)})) + H(P ({\rmY \mid  \psi(\rmY)}))$ & \\ 
\textbf{GReg1} & $ \KL(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})] \Vert \mathcal{O}))$  \\ 
\textbf{iAim1} &  $H(\mathbb{E}[ P ({\phi(\rmX_n)})])$ & \\ 
\textbf{GAim1} &  $ H(\mathbb{E}[ P ({\phi(\rmX_n), \rmY_n})])$  \\
 \textbf{iReg2} & $ -H(\mathbb{E}[ P ({\phi(\rmX_n)})]) + H(P({\phi(\rmX)}))$ & \\ 
 \textbf{GReg2} & ${ - H(P(\phi(\rmX)  \mid  \psi(\rmY))) 
+ H(P(\phi(\rmX)))}$ \\  
\bottomrule
\end{tabular}%
% }
\caption{Notations for terms in the paper (above) and its derived formulation (below) in the appendix.}
\label{tab:note_align}
\end{table}



\section{Experimental Details and Parameters}
\label{app:para}
\textbf{We have conducted  $248$ experiments in total,} including 
$12$ Toy experiments (training $3$ objective settings on $4$ domain settings), 
$20$ Regression experiments in Monocular depth estimation (training $5$ objective settings on $4$ domain settings), 
$9$ Segmentation experiments (training $3$ objective settings on $1$ domain settings and verifying on $3$ domain settings), 
$63$ Classification experiments (training $1$ objective settings on $5$ datasets that has $4,4,4,4,5$ domain settings for $3$ trails), 
and $144$ ablation study experiments (training $12$ objective settings on $1$ dataset that has $4$ domain settings for $3$ trails).
% \textbf{There are $248$ experiments in total.}
We believe that the consistent improvements yielded by GMDG in these experiments validate the superiority of our GMDG.


Experimental details of these experiments can be found in the following.
Note that we set $v_{A2} = 1$  for all experiments. 

\subsection{Toy experiments: Synthetic regression experimental details.}
We explore the efficacy of $\psi$ by using toy regression experiments with synthetic data.

\textbf{Datasets.} The latent features in all three domains are added some distributional shifts and used as the first group in the raw features (denoted as $x^1_n, y^1_n$ where $n\in{1,2,3}$ represent which domain it belongs to). Then, some domain-conditioned transformations are applied to shifted features, or some pure random noises are used as the second group in the raw features (denoted as $x^2_n, y^2_n$). 
Therefore the constructed 
$X_{n\in\{1,2,3\}}= [x^1_n, x^2_n], Y_{n\in\{1,2,3\}} = [y^1_n,y^2_n]$  both contain features that dependents on $D$. 
Details of each synthetic data are exhibited in Table~\ref{tab:syn}. We generate $10000$ samples for training and $100$ samples for validation and testing sets.

\textbf{Parameter settings.} All experiments are conducted with $v_{A1}, v_{R1}, v_{R2}= 0.1$.

\textbf{Experimental settings.} For $\phi,\psi$, we use three-layer MLP and one linear layer for regression prediction and Mean Squared Error (MSE) as the loss. We use the best model on the validation dataset for testing. 

\textbf{Metric.} We use the MSE between the predictions and the $Y$ of the testing set as the evaluation metric.


\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{toy.pdf}
    \caption{Toy experiments: Diagram of constructing the toy dataset. 
    % \red{need fix}
    }
    \label{fig:toy_figure}
\end{figure*}




\begin{table*}[t]
\centering
\begin{tabular}{lllll}
\toprule
$hx$ & $hx \sim \mathcal{N}(hx; 0, 1)$ \\
$hy$ & $hy= hx$ \\  \midrule 
Data 1 & Without distribution shift & With affine transformations \\
$X_1$ & $x_1^1 =hx$ & $x_1^2 = x_1^1 +\epsilon\sim \mathcal{N}(\epsilon; 0, 0.3)$ &  \\
$Y_1$ & $y_1^1 =hy$ & $y_1^2 = y_1^1 +\epsilon\sim \mathcal{N}(\epsilon; 0, 0.3)$ &  \\ \hline
$X_2$ & $x_2^1 =hx$ & $x_2^2 = 4 \times x_2^1 + \epsilon \sim \mathcal{N}(\epsilon; 0.5, 0.3)$ &  \\
$Y_2$ & $y_2^1 =hy$ & $y_2^2 = 4 \times y_2^1 + 0.3 $ &  \\ \hline
$X_3$ & $x_3^1 =hx$ & $x_3^2 = 2 \times x_3^1 + \epsilon \sim \mathcal{N}(\epsilon; -0.3, 0.2)$ &  \\
$Y_3$ & $y_3^1 =hy$ & $y_3^2 = 0.5 \times y_3^1 - 0.2$ &  \\
\midrule 
Data 2 & With distribution shift &  With affine transformations \\
$X_1$ & $x_1^1 =hx$ & $x_1^2 = x_1^1 +\epsilon\sim \mathcal{N}(\epsilon; 0, 0.3)$ &  \\
$Y_1$ & $y_1^1 =hy$ & $y_1^2 = y_1^1+\epsilon\sim \mathcal{N}(\epsilon; 0, 0.3)$ &  \\ \hline
$X_2$ & $x_2^1 =hx+\epsilon\sim \mathcal{N}(\epsilon; -0.1, 0.1)$ & $x_2^2 = 4 \times x_2^1 + \epsilon \sim \mathcal{N}(\epsilon; 0.3, 0.3)$ &  \\
$Y_2$ & $y_2^1 =hy+\epsilon\sim \mathcal{N}(\epsilon; 0.2, 0.1)$  & $y_2^2 = 8 \times y_2^1 - 0.3 $ &  \\ \hline
$X_3$ & $x_3^1 =hx+\epsilon\sim \mathcal{N}(\epsilon; 0.4, 0.2)$  & $x_3^2 = -1 \times x_3^1 +\epsilon \sim \mathcal{N}(\epsilon; -0.3, 0.2)$ &  \\
$Y_3$ & $y_3^1 =hy+\epsilon\sim \mathcal{N}(\epsilon; -0.4, 0.2)$ & $y_3^2 = \epsilon \sim \mathcal{N}(\epsilon; 0, 0.2)$ & 
\\
\midrule 
Data 3 & Without distribution shift & With squared, cubed transformations or noises\\
$X_1$ & $x_1^1 =hx$ & $x_1^2 = x_1^1 +\epsilon\sim \mathcal{N}(\epsilon; 0, 0.3)$ &  \\
$Y_1$ & $y_1^1 =hy$ & $y_1^2 = y_1^1+\epsilon\sim \mathcal{N}(\epsilon; 0, 0.3)$ &  \\ \hline
$X_2$ & $x_2^1 =hx$ & $x_2^2 = 4 \times x_2^1 ** 3 + \epsilon \sim \mathcal{N}(\epsilon; 0.5, 0.3)$ &  \\
$Y_2$ & $y_2^1 =hy$ & $y_2^2 = 4 \times y_2^1 ** 2 + 0.3 $ &  \\ \hline
$X_3$ & $x_3^1 =hx$ & $x_3^2 = 2 \times x_3^1 ** 2 +\epsilon \sim \mathcal{N}(\epsilon; -0.3, 0.2)$ &  \\
$Y_3$ & $y_3^1 =hy$ & $y_3^2 = 0.5 \times y_3^1 ** 3 - 0.2 $ & 
\\
\midrule 
Data 4 & With distribution shift & With squared, cubed transformations or noises\\ 
$X_1$ & $x_1^1 =hx$ & $x_1^2 = x_1^1 +\epsilon\sim \mathcal{N}(\epsilon; 0, 0.3)$ &  \\
$Y_1$ & $y_1^1 =hy$ & $y_1^2 = y_1^1+\epsilon\sim \mathcal{N}(\epsilon; 0, 0.3)$ &  \\ \hline
$X_2$ & $x_2^1 =hx+\epsilon\sim \mathcal{N}(\epsilon; -0.1, 0.1)$ & $x_2^2 = 4 \times x_2^1 ** 3 + \epsilon \sim \mathcal{N}(\epsilon; 0.5, 0.3)$ &  \\
$Y_2$ & $y_2^1 =hy+\epsilon\sim \mathcal{N}(\epsilon; 0.2, 0.1)$  & $y_2^2 = 4 \times y_2^1 ** 2 + 0.3 $ &  \\ \hline
$X_3$ & $x_3^1 =hx+\epsilon\sim \mathcal{N}(\epsilon; 0.4, 0.2)$  & $x_3^2 = 2 \times x_3^1 ** 2 +\epsilon \sim \mathcal{N}(\epsilon; -0.3, 0.2)$ &  \\
$Y_3$ & $y_3^1 =hy+\epsilon\sim \mathcal{N}(\epsilon; -0.4, 0.2)$ & $y_3^2 = 0.5 \times y_3^1 ** 3 - 0.2 $ & \\
\bottomrule
\end{tabular}
\caption{Toy experiments: Synthetic data details for each experiment.}
\label{tab:syn}
\end{table*}
\begin{table*}[t]
    \centering
    \begin{tabular}{lccccccccc}
        \toprule
         Use ResNet-50 without SWAD &  $v2$  & $v3$ & $v1$  & lr mult & lr & dropout & WD & TR & CF \\ \hline
         TerraIncognita &  0.1 & 0.1 &  0.2 &  12.5 & - & - & - & - & - \\
         OfficeHome & 0.1 &  0.001 & 0.1 & 20.0 & 3e-5 & 0.1 & 1e-6 & - & - \\
         VLCS & 0.01 & 0.001 & 0.1 & 10.0 & 1e-5 & - & 1e-6 & 0.2 & 50 \\
         PACS & 0.01 & 0.01 & 0.01 & 25.0 & - & - & - & - & -   \\
         DomainNet & 0.1 & 0.1 & 0.1 & 7.5 & - & - & - & - & 500
         \\ \bottomrule 
         \\
    \end{tabular}

    \begin{tabular}{lccccccccc}
    \toprule
         Use ResNet-50 with SWAD & $v2$  & $v3$ & $v1$  & lr mult & CF \\ \hline
         TerraIncognita &  0.1 & 0.001 &  0.01 &  10.0 & - \\
         OfficeHome & 0.1 &  0.1 & 0.3 & 10.0 &  - \\
         VLCS & 0.01 & 0.001 & 0.1 & 10.0 &  50 \\
         PACS & 0.01 & 0.001 & 0.1 & 20.0 & -   \\ 
         DomainNet & 0.1 & 0.1 & 0.1 & 7.5 & 500 \\
    \bottomrule \\
    \end{tabular}

    \begin{tabular}{lccccccccc}
    \toprule
         Use RegNetY-16GF with and without SWAD & $v2$  & $v3$ & $v1$  & lr mult & CF \\ \hline
         TerraIncognita &  0.01 & 0.01 &  0.01 & 2.5 & - \\
         OfficeHome & 0.01 &  0.1 & 0.1 & 0.1 &  - \\
         VLCS & 0.01 &  0.01  & 0.1 & 2.0 &  50 \\
         PACS & 0.01 & 0.1 & 0.1 & 0.1 & -   \\ 
         DomainNet & 0.1 & 0.1 & 0.1 & 7.5 & 500 \\
    \bottomrule     
    \end{tabular}
  \caption{Classification experiments: Parameter settings of classification tasks. Notations: WD: weight decay; TR: tolerance ratio; CF: checkpoint freq. - denotes that for where the default settings are used.}
    \label{tab:main_para}
\end{table*}
\begin{table*}[t]
    \centering
     \begin{tabular}{lccccccccc}
    \toprule
         Ablation studies on OfficeHome& $v2$  & $v3$ & $v1$  & lr mult  & use \textbf{iAim1} & use \textbf{iReg2} \\ \hline
        {Base} (ERM) & 0.0 &  0.0 & 0.0 & 0.1 &  False & False\\
        {Base +iAim1} (DANN) & 0.0 &  0.0 & 0.1 & 0.1 &  True & False\\
        {Base + GAim1} (CDANN, CIDG)  & 0.0 &  0.0 & 0.1 & 0.1 &  False & False\\
        {Base  +iReg2} (CORAL+$\psi$) & 0.0 &  0.1 & 0.0 & 0.1 &  False & True\\
        {Base + GReg2} & 0.0 &  0.1 & 0.0 & 0.1 &  False & False\\
        {Base + GAim1 + GReg2} (MDA+$\psi$) & 0.0 &  0.1 & 0.1 & 0.1 &  False & False\\
        {Base + GReg1} (MIRO, SIMPLE) & 0.01 &  0.0 & 0.0 & 0.1 &  False & False\\
        {Base + GReg1 +iAim1} & 0.01 &  0.0 & 0.1 & 0.1 &  False & True\\
        {Base + GReg1 + GAim1} & 0.01 &  0.0 & 0.1 & 0.1 &  False & False\\
        {Base + GReg1 +iReg2} & 0.01 &  0.1 & 0.0 & 0.1 &  True & False\\
        {Base + GReg1 + GReg2} & 0.01 &  0.1 & 0.0 & 0.1 &  False & False\\
        {Base + GReg1 + GAim1 + GReg2 (Ours)} & 0.01 &  0.1 & 0.1 & 0.1 &  False & False\\
    \bottomrule   
    \end{tabular}
\caption{Ablation studies: Parameter settings of ablation studies. Notations: WD:  CF: checkpoint freq. - denotes that for where the default settings are used.}
\label{tab:ablation_para}
\end{table*}

\subsection{Regression experiments: Monocular depth estimation details.}
We explore the efficacy of $\psi$ with GMDG by using toy monocular depth estimation experiments with NYU Depth V2 dataset~\cite{silberman2012indoor}. 


\textbf{Datasets.}
NYU Depth
V2 contains images with  $480 \times 640$  resolution with depth values ranging from 0 to 10 meters. We adopt the densely labeled pairs for training and testing.


\textbf{Multi-domain construction.} To construct multiple domains that fit the problem settings, we split the NYU Depth V2 dataset into four categories as four domains:
\begin{itemize}
    \item {School}: study room,
            study,
            student lounge,
            printer room,
            computer lab,
            classroom.
     \item {Office}: reception room,
            office kitchen,
            office,
            nyu office,
            conference room.
     \item {Home}: playroom,
            living room,
            laundry room,
            kitchen,
            indoor balcony,
            home storage,
            home office,
            foyer,
            dining room,
            dinette,
            bookstore,
            bedroom,
            bathroom,
            basement.
    \item {Commercial}:furniture store,
            exercise room,
            cafe.
\end{itemize}
After filtering data samples that are not able to be used, each domain has $95$, $110$, $1209$, and $35$ data pairs that can be used for training. 

\textbf{Parameter settings.} We follow all the hyperparameter settings in the VA-DepthNet and set $v_{A1} =0.001, v_{R1} = 0.001, v_{R2} = 0.0001$.  Note that the backbone is trained using VA-DepthNet but without the Variational Loss proposed by VA-DepthNet. 

\textbf{Experimental settings.} We use the final saved checkpoint for the leave-one-out cross-validation. 

\textbf{Metrics.} Please see metric details in VA-DepthNet~\cite{liu2023va}.



\subsection{Segmentation experimental details.}
We follow the experimental settings of RobustNet for segmentation experiments.

% To verify the generalization capability of our methods, we
% conduct the experiments on five different datasets.
\textbf{Datasets.} There are two groups of datasets: Synthetic datasets and real-world datasets.
(1) Synthetic datasets: GTAV~\cite{richter2016gtav} is a large-scale dataset containing 24,966 driving-scene images generated from the Grand Theft Auto V game engine. SYNTHIA~\cite{ros2016synthia} which is composed of photo-realistic synthetic images has 9,400 samples with a resolution of 960×720.
% It has 12,403, 6,382, and
% 6,181 images of size 1914×1052 for a train, a validation,
% and a test set, respectively, containing 19 object categories. 
% compatible with Cityscapes. 
% Also, we use SYNTHIA [50], composed of photo-realistic synthetic images containing 9,400
% samples with a resolution of 960×720.
(2) Real-world datasets: Cityscapes~\cite{cordts2016cityscapes} is a large-scale dataset containing high-resolution urban scene images. 
Providing 3,450 finely annotated images and 20,000 coarsely annotated images, it collects data from 50 different cities in primarily Germany. Only the finely annotated set is adopted for our training and validation. BDD-100K~\cite{yu2020bdd100k} is
another real-world dataset with a resolution of 1280×720. It provides diverse urban driving scene images from various locations in the US. We use the 7,000 training and 1,000 validation of the semantic segmentation task.
The images are collected from various locations in the US. 
% For a
% semantic segmentation task, 7,000 training and 1,000 validation images are provided. 
Mapillary is also a real-world dataset that contains worldwide street-view scenes with 25,000 high-resolution images. 
% The last real-world dataset we
% use is Mapillary [42], a diverse street-view dataset consisting of 25,000 high-resolution images with a minimum resolution of 1920×1080 collected from all around the world.


\textbf{Parameter settings.} Specifically, we use all RobustNet's hyper-parameters and set $v_{A1} = 0.0001, v_{R1} = 0.0001$.


\subsection{Classification experimental details.} 

% Note here `d\_shift' is the weight $v_1$ of $\mathcal{L}_{A1}$, `ld' is the weight $v_2$ of $\mathcal{L}_{T2}$ and `shift' is the weight $v_3$ of $\mathcal{L}_{T3}$. 

\textbf{Datasets.}
We use PACS (4 domains, 9,991
samples, $7$ classes)~\citep{li2017deeper}, VLCS ($4$ domains, $10,729$ samples, $5$ classes)~\citep{fang2013unbiased}, OfficeHome (4 domains, 15,588 samples, 65 classes)~\citep{venkateswara2017deep}, TerraIncognita (TerraInc, $4$ domains, $24,778$ samples, $10$ classes)~\citep{beery2018recognition}, and DomainNet (6 domains,
586,575 samples, 345 classes)~\citep{peng2019moment}.




\textbf{Parameter settings.}  We list the hyper-parameters in Table~\ref{tab:main_para} to reproduce our results.

\textbf{Metric.} We employ mean
Intersection over Union (mIoU) as the measurement for the segmentation task.
% For all the quantitative experiments, mean
% Intersection over Union (mIoU) is used to measure the segmentation performance.

% {Use ResNet-50 without SWAD:}


% \begin{scriptsize}
% \begin{lstlisting}
% --dataset TerraIncognita --ld 0.1 --shift 0.1 --d_shift 0.2 --lr_mult 12.5
% --dataset OfficeHome --ld 0.1 --lr 3e-5 --resnet_dropout 0.1 --weight_decay 1e-6 --ld 0.1 --shift 0.001 --d_shift 0.1 --lr_mult 20.0
% --dataset VLCS --checkpoint_freq 50 --tolerance_ratio 0.2 --lr 1e-5 --resnet_dropout 0.5 --weight_decay 1e-6 --ld 0.01 --shift 0.001 --d_shift 0.1 --lr_mult 10 
% --dataset PACS --ld 0.01 --shift 0.01 --d_shift 0.01 --lr_mult 25.
% --dataset DomainNet --ld 0.1 --checkpoint_freq 500 --shift 0.1 --d_shift 0.1 --lr_mult 7.5
% \end{lstlisting}
% \end{scriptsize}

% {Use ResNet-50 with SWAD:}
% \begin{scriptsize}
% \begin{lstlisting}
% --dataset TerraIncognita --ld 0.1 --swad True --shift 0.001 --d_shift 0.01 --lr_mult 10
% --dataset OfficeHome --swad True --ld 0.1 --shift 0.1 --d_shift 0.3 --lr_mult 10.
% --dataset VLCS --checkpoint_freq 50 --tolerance_ratio 0.2 --ld 0.01 --swad True --swad True --shift 0.001 --d_shift 0.1 --lr_mult 10.
% --dataset PACS --ld 0.01 --swad True --shift 0.001 --d_shift 0.1 --lr_mult 20.
% --dataset DomainNet --ld 0.1 --checkpoint_freq 500 --swad True --shift 0.1 --d_shift 0.1 --lr_mult 7.5
% \end{lstlisting}
% \end{scriptsize}

% {Use RegNetY-16GF with and without SWAD}
% \begin{scriptsize}
% \begin{lstlisting}
% --dataset TerraIncognita --ld 0.01 --model swag_regnety_16gf --batch_size 16 --checkpoint_freq 200 --swad True --shift 0.01 --d_shift 0.01 --lr_mult 2.5
% --dataset OfficeHome --ld 0.01 --model swag_regnety_16gf --batch_size 16 --swad True --shift 0.1 --d_shift 0.1 --lr_mult 0.1
% --dataset VLCS --ld 0.01 --checkpoint_freq 50 --tolerance_ratio 0.2 --model swag_regnety_16gf --batch_size 16 --swad True --shift 0.01 --d_shift 0.1 --lr_mult 2.
% --dataset PACS --ld 0.01 --model swag_regnety_16gf --batch_size 16 --swad True --shift 0.1 --d_shift 0.1 --lr_mult 0.1
% --dataset DomainNet --ld 0.1 --checkpoint_freq 500 --model swag_regnety_16gf --batch_size 14 --swad True --shift 0.1 --d_shift 0.1
% \end{lstlisting}
% \end{scriptsize}


\subsection{Ablation studies experimental details.} 

% All experiments are using the 


\textbf{Parameter settings.} We run each experiment in three trials with seeds: $[0, 1, 2]$.  Full settings are reported in Table~\ref{tab:ablation_para}.
Especially,

\textbf{Experimental settings.} We use SWAD for all ablation studies to alleviate the effeteness of hyper-parameters. All ablation studies share the same hyper-parameters but add different combinations of terms. CORAL's~\citep{sun2016deep} objective focuses on minimizing the learned feature covariance discrepancy between source and target, requiring target data access and only regards second-order statistics. We adapt its approach to minimize feature covariances across seen domains for a fair comparison. 
% \begin{scriptsize}
% \begin{lstlisting}
% --dataset OfficeHome --ld 0.01 --model swag_regnety_16gf --batch_size 16 --swad True --shift -0.1 --d_shift 0.1 --lr_mult 0.1 --trial_seed 0 --use_condition1 Ture --use_condition2 Ture
% \end{lstlisting}
% \end{scriptsize}


% \begin{table}[h]
%     \centering
%     \caption{Segmentation experiments +$\mathcal{L}_{A1}$: mIoU results of Cityscapes}
%     \label{tab:seg_t1_cityscapes}
%     \begin{tabular}{lllllllllllllll}
% label id  &    label  &  iU     &  Precision &   Recall &  TP     &   FP      &   FN  \\ \hline
%  0        &        0  &  77.9   &    0.8     &     0.9  &   30.6  &      0.2  &   0.1  \\
%  1        &        1  &  33.1   &    0.7     &     0.4  &    3.7  &      0.5  &   1.5  \\
%  2        &        2  &  79.6   &    0.9     &     0.8  &   20.3  &      0.1  &   0.2  \\
%  3        &        3  &  25.9   &    0.3     &     0.6  &    0.2  &      2.3  &   0.6  \\
%  4        &        4  &   6.7   &    0.1     &     0.7  &    0.1  &     13.5  &   0.4  \\
%  5        &        5  &  33.0   &    0.4     &     0.7  &    0.6  &      1.5  &   0.5  \\
%  6        &        6  &  19.6   &    0.2     &     0.9  &    0.0  &      4.0  &   0.1  \\
%  7        &        7  &  28.2   &    0.3     &     0.8  &    0.2  &      2.4  &   0.2  \\
%  8        &        8  &  82.9   &    0.9     &     0.9  &   16.0  &      0.1  &   0.1  \\
%  9        &        9  &  29.6   &    0.3     &     0.7  &    0.3  &      2.0  &   0.3  \\
% 10        &       10  &  80.5   &    1.0     &     0.8  &    3.3  &      0.0  &   0.2  \\
% 11        &       11  &  61.5   &    0.8     &     0.7  &    1.0  &      0.3  &   0.3  \\
% 12        &       12  &  24.5   &    0.4     &     0.4  &    0.1  &      1.6  &   1.5  \\
% 13        &       13  &  72.0   &    0.9     &     0.8  &    6.1  &      0.1  &   0.3  \\
% 14        &       14  &  12.8   &    0.1     &     0.7  &    0.0  &      6.3  &   0.5  \\
% 15        &       15  &  32.4   &    0.7     &     0.4  &    0.3  &      0.5  &   1.6  \\
% 16        &       16  &   0.0   &    0.0     &     0.3  &    0.0  &    10315.5&   2.1  \\
% 17        &       17  &  10.5   &    0.1     &     0.7  &    0.0  &      8.1  &   0.4  \\
% 18        &       18  &  23.9   &    0.2     &     0.9  &    0.2  &      3.1  &   0.1  \\ \hline
% mean & 0.3867
%     \end{tabular}
% \end{table}

% \begin{table}[h]
%     \centering
%     \caption{Segmentation experiments +$\mathcal{L}_{A1}$: mIoU results of Cityscapes}
%     \label{tab:seg_t1_cityscapes}
%     \begin{tabular}{lllllllllllllll}
% label id    &  label   &   iU     & Precision & Recall  & TP      & FP       &  FN \\  \hline
%  0          &      0   &   75.0   &   0.8     &   0.9   &  20.0   &    0.2   &    0.1 \\
%  1          &      1   &   32.1   &   0.6     &   0.4   &   1.3   &    0.8   &    1.3 \\
%  2          &      2   &   73.7   &   0.9     &   0.8   &  15.0   &    0.1   &    0.2 \\
%  3          &      3   &   10.4   &   0.1     &   0.4   &   0.1   &    6.8   &    1.8 \\
%  4          &      4   &   19.7   &   0.2     &   0.8   &   0.2   &    3.8   &    0.2 \\
%  5          &      5   &   28.4   &   0.4     &   0.6   &   0.4   &    1.8   &    0.7 \\
%  6          &      6   &   24.4   &   0.3     &   0.8   &   0.0   &    2.8   &    0.3 \\
%  7          &      7   &   22.8   &   0.3     &   0.7   &   0.1   &    2.9   &    0.5 \\
%  8          &      8   &   74.9   &   0.9     &   0.8   &  15.5   &    0.2   &    0.2 \\
%  9          &      9   &   23.8   &   0.3     &   0.5   &   0.3   &    2.3   &    0.9 \\
% 10          &     10   &   89.4   &   0.9     &   1.0   &  19.3   &    0.1   &    0.0 \\
% 11          &     11   &   47.0   &   0.6     &   0.7   &   0.2   &    0.7   &    0.5 \\
% 12          &     12   &   17.6   &   0.4     &   0.2   &   0.0   &    1.5   &    3.2 \\
% 13          &     13   &   62.0   &   0.9     &   0.7   &   9.8   &    0.1   &    0.5 \\
% 14          &     14   &   13.1   &   0.2     &   0.5   &   0.2   &    5.6   &    1.0 \\
% 15          &     15   &   38.2   &   0.6     &   0.5   &   0.4   &    0.6   &    1.0 \\
% 16          &     16   &    0.0   &   0.0     &   0.0   &   0.0   &    inf   &    inf \\
% 17          &     17   &   20.3   &   0.2     &   0.8   &   0.0   &    3.7   &    0.3 \\
% 18          &     18   &   21.2   &   0.2     &   0.7   &   0.0   &    3.3   &    0.4 \\  \hline
% mean & 0.3652
%     \end{tabular}
% \end{table}

% \begin{table}[h]
%     \centering
%     \caption{Segmentation experiments +$\mathcal{L}_{A1}$: mIoU results of Cityscapes}
%     \label{tab:seg_t1_cityscapes}
%     \begin{tabular}{lllllllllllllll}
%     label id   &   label  &   iU    & Precision &  Recall & TP     &  FP      &FN \\ \hline
%  0         &       0  &   78.0  &   0.8     &    0.9  &  20.8  &     0.2  &     0.1 \\
%  1         &       1  &   38.5  &   0.6     &    0.5  &   2.7  &     0.6  &     1.0 \\
%  2         &       2  &   72.7  &   0.9     &    0.8  &  10.8  &     0.1  &     0.3 \\
%  3         &       3  &   19.0  &   0.2     &    0.5  &   0.2  &     3.3  &     1.0 \\
%  4         &       4  &   13.5  &   0.1     &    0.7  &   0.2  &     6.0  &     0.4 \\
%  5         &       5  &   35.1  &   0.4     &    0.7  &   0.6  &     1.4  &     0.5 \\
%  6         &       6  &   23.0  &   0.2     &    0.9  &   0.0  &     3.2  &     0.1 \\
%  7         &       7  &   45.2  &   0.5     &    0.9  &   0.3  &     1.0  &     0.2 \\
%  8         &       8  &   78.5  &   0.8     &    0.9  &  12.7  &     0.2  &     0.1 \\
%  9         &       9  &   40.4  &   0.6     &    0.5  &   0.7  &     0.6  &     0.9 \\
% 10         &      10  &   94.3  &   1.0     &    1.0  &  34.0  &     0.0  &     0.0 \\
% 11         &      11  &   59.9  &   0.8     &    0.7  &   0.2  &     0.3  &     0.4 \\
% 12         &      12  &   27.9  &   0.4     &    0.5  &   0.0  &     1.7  &     0.8 \\
% 13         &      13  &   64.8  &   0.9     &    0.7  &   3.1  &     0.1  &     0.5 \\
% 14         &      14  &   17.1  &   0.2     &    0.7  &   0.1  &     4.5  &     0.4 \\
% 15         &      15  &   19.0  &   0.6     &    0.2  &   0.1  &     0.8  &     3.5 \\
% 16         &      16  &    0.1  &   0.0     &    0.0  &   0.0  &   736.2  &   257.6 \\
% 17         &      17  &   12.4  &   0.1     &    0.8  &   0.0  &     6.8  &     0.3 \\ 
% 18         &      18  &   24.9  &   0.3     &    0.7  &   0.0  &     2.6  &     0.4 \\ \hline
% mean & 0.4023
%     \end{tabular}
% \end{table}

\section{More results}
\label{app:res}


% \begin{table*}[t]
% % \centering
% \caption{Main results: the proposed method compared with previous non-ensemble and ensemble mDG methods. The best results for each group are highlighted in \textbf{bold}.
% % and \textbf{\textit{italic}}, respectively.
% % \red{cite}
% }
% % \label{tab:main_res1}
% \begin{center}
% \small
% \begin{tabular}{p{4.15cm}cccccp{0.4cm}}
%  \hline  \hline 
% & \multicolumn{6}{c}{\bf Non-ensemble methods} \\ 
%  & \bf PACS & \bf VLCS & \bf OfficeHome & \bf TerraInc & \bf DomainNet & \bf Avg. \\ \hline
%  % & \multicolumn{6}{c}{\bf No oracle model.} \\ 
% MMD~\citep{li2018domainMMD} & 84.7±0.5 & 77.5±0.9 & 66.3±0.1 & 42.2±1.6 & 23.4±9.5 & 58.8 \\
% Mixstyle~\citep{zhou2021domain} & 85.2±0.3 & 77.9±0.5 & 60.4±0.3 & 44.0±0.7 & 34.0±0.1 & 60.3 \\
% GroupDRO~\citep{sagawa2019distributionally} & 84.4±0.8 & 76.7±0.6 & 66.0±0.7 & 43.2±1.1 & 33.3±0.2 & 60.7 \\
% IRM~\cite{arjovsky2019invariant} & 83.5±0.8 & 78.5±0.5 & 64.3±2.2 & 47.6±0.8 & 33.9±2.8 & 61.6 \\
% ARM~\citep{zhang2021adaptive} & 85.1±0.4 & 77.6±0.3 & 64.8±0.3 & 45.5±0.3 & 35.5±0.2 & 61.7 \\
% VREx~\citep{krueger2021out} & 84.9±0.6 & 78.3±0.2 & 66.4±0.6 & 46.4±0.6 & 33.6±2.9 & 61.9 \\
% CDANN~\citep{li2018deep} & 82.6±0.9 & 77.5±0.1 & 65.8±1.3 & 45.8±1.6 & 38.3±0.3 & 62.0 \\
% DANN~\citep{ganin2016domain} & 83.6±0.4 & 78.6±0.4 & 65.9±0.6 & 46.7±0.5 & 38.3±0.1 & 62.6 \\
% RSC~\citep{huang2020self} & 85.2±0.9 & 77.1±0.5 & 65.5±0.9 & 46.6±1.0 & 38.9±0.5 & 62.7 \\
% MTL~\citep{blanchard2021domain} & 84.6±0.5 & 77.2±0.4 & 66.4±0.5 & 45.6±1.2 & 40.6±0.1 & 62.9 \\
% % Mixup & 84.6±0.6 & 77.4±0.6 & 68.1±0.3 & 47.9±0.8 & 39.2±0.1 & 63.4 \\
% MLDG~\citep{li2018learning} & 84.9±1.0 & 77.2±0.4 & 66.8±0.6 & 47.7±0.9 & 41.2±0.1 & 63.6 \\
% Fish~\citep{shi2021gradient} & 85.5±0.3 & 77.8±0.3 & 68.6±0.4 & 45.1±1.3 & 42.7±0.2 & 63.9 \\
% ERM~\citep{Vapnik1998ERM} & 84.2±0.1 & 77.3±0.1 & 67.6±0.2 & 47.8±0.6 & 44.0±0.1 & 64.2 \\
% SagNet~\citep{nam2021reducing} & \textbf{86.3}±0.2 & 77.8±0.5 & 68.1±0.1 & 48.6±1.0 & 40.3±0.1 & 64.2 \\
% SelfReg~\citep{kim2021selfreg} & 85.6±0.4 & 77.8±0.9 & 67.9±0.7 & 47.0±0.3 & 42.8±0.0 & 64.2 \\
% CORAL~\citep{sun2016deep} & 86.2±0.3 & 78.8±0.6 & 68.7±0.3 & 47.6±1.0 & 41.5±0.1 & 64.5 \\
% mDSDI~\cite{bui2021exploiting} & 86.2±0.2 & 79.0±0.3 & 69.2±0.4 & 48.1±1.4 & 42.8±0.1 & 65.1 \\ 
% % MDA~\cite{} &  - &  70.2 & -  & -  & - & - \\ 
%  & \multicolumn{6}{c}{Use ResNet-50~\citep{he2016deep} as oracle model.} \\ 
% MIRO~\citep{cha2022miro}  & 85.4±0.4 & 79.0±0.3 & 70.5±0.4 & 50.4±1.1 & 44.3±0.2 & 65.9 \\ 
% \textbf{Ours} & 85.6±0.3 & \textbf{79.2}±0.3 &\textbf{70.7}±0.2 & \textbf{51.1}±0.9 & \textbf{44.6}±0.1 & \textbf{66.3} \\ \hline
%  & \multicolumn{6}{c}{Use RegNetY-16GF~\citep{singh2022revisiting} as oracle model.} \\ 
% MIRO  & \textbf{97.4}±0.2 & 79.9±0.6 & 80.4±0.2 & 58.9±1.3 & 53.8±0.1 & 74.1 \\
% \textbf{Ours} & 97.3±0.1 & \textbf{82.4}±0.6 & \textbf{80.8}±0.6 & \textbf{60.7}±1.8 & \textbf{54.6}±0.1 & \textbf{75.1} \\ \hline  \hline
% & \multicolumn{6}{c}{\bf Ensemble methods} \\ 
%  & \bf PACS & \bf VLCS & \bf OfficeHome & \bf TerraInc & \bf DomainNet & \bf Avg. \\ \hline
% & \multicolumn{6}{c}{ Use multiple oracle models.} \\ 
% % \hline
% SIMPLE~\citep{li2022simple} & 88.6±0.4 & 79.9±0.5 & 84.6±0.5 & 57.6±0.8 & 49.2±1.1 & 72.0 \\
% SIMPLE++~\citep{li2022simple} & \textbf{99.0}±0.1 & \textbf{82.7}±0.4 & \textbf{87.7}±0.4 & \textbf{59.0}±0.6 & \textbf{61.9}±0.5 & \textbf{{78.1}} \\ \hline 
% % \hline
%  % & \multicolumn{6}{c}{\bf No oracle model.} \\ 
% % MMD & 84.7±0.5 & 77.5±0.9 & 66.3±0.1 & 42.2±1.6 & 23.4±9.5 & 58.8 \\
% % Mixstyle & 85.2±0.3 & 77.9±0.5 & 60.4±0.3 & 44.0±0.7 & 34.0±0.1 & 60.3 \\
% % GroupDRO & 84.4±0.8 & 76.7±0.6 & 66.0±0.7 & 43.2±1.1 & 33.3±0.2 & 60.7 \\
% % IRM & 83.5±0.8 & 78.5±0.5 & 64.3±2.2 & 47.6±0.8 & 33.9±2.8 & 61.6 \\
% % ARM & 85.1±0.4 & 77.6±0.3 & 64.8±0.3 & 45.5±0.3 & 35.5±0.2 & 61.7 \\
% % VREx & 84.9±0.6 & 78.3±0.2 & 66.4±0.6 & 46.4±0.6 & 33.6±2.9 & 61.9 \\
% % CDANN & 82.6±0.9 & 77.5±0.1 & 65.8±1.3 & 45.8±1.6 & 38.3±0.3 & 62.0 \\
% % DANN & 83.6±0.4 & 78.6±0.4 & 65.9±0.6 & 46.7±0.5 & 38.3±0.1 & 62.6 \\
% % RSC & 85.2±0.9 & 77.1±0.5 & 65.5±0.9 & 46.6±1.0 & 38.9±0.5 & 62.7 \\
% % MTL & 84.6±0.5 & 77.2±0.4 & 66.4±0.5 & 45.6±1.2 & 40.6±0.1 & 62.9 \\
% % Mixup & 84.6±0.6 & 77.4±0.6 & 68.1±0.3 & 47.9±0.8 & 39.2±0.1 & 63.4 \\
% % MLDG & 84.9±1.0 & 77.2±0.4 & 66.8±0.6 & 47.7±0.9 & 41.2±0.1 & 63.6 \\
% % Fish & 85.5±0.3 & 77.8±0.3 & 68.6±0.4 & 45.1±1.3 & 42.7±0.2 & 63.9 \\
% % ERM & 84.2±0.1 & 77.3±0.1 & 67.6±0.2 & 47.8±0.6 & 44.0±0.1 & 64.2 \\
% % SagNet & 86.3±0.2 & 77.8±0.5 & 68.1±0.1 & 48.6±1.0 & 40.3±0.1 & 64.2 \\
% % SelfReg & 85.6±0.4 & 77.8±0.9 & 67.9±0.7 & 47.0±0.3 & 42.8±0.0 & 64.2 \\
% % CORAL & 86.2±0.3 & 78.8±0.6 & 68.7±0.3 & 47.6±1.0 & 41.5±0.1 & 64.5 \\
% % mDSDI & 86.2±0.2 & 79.0±0.3 & 69.2±0.4 & 48.1±1.4 & 42.8±0.1 & 65.1 \\ \hline 
% & \multicolumn{6}{c}{Use ResNet-50~\citep{he2016deep} as oracle model.} \\ 
% % \hline
% % MIRO  & 85.4±0.4 & 79.0±0.3 & 70.5±0.4 & 50.4±1.1 & 44.3±0.2 & 65.9 \\ 
% % \textbf{Ours} & \textbf{85.6}±0.3 & \textbf{79.2}±0.3 & \textbf{70.7}±0.2 & \textbf{51.1}±0.9 & \textbf{44.6}±0.1 & \textbf{66.3} \\ \hline
% % & \blue{+0.2} &  \blue{+0.1} &  \blue{+0.2} &  \blue{+0.7} &  \blue{+0.3} &   \blue{+0.3}\\ 
% MIRO + SWAD  &  \textbf{88.4}±0.1 & {{79.6}}±0.2 & {{72.4}}±0.1 & {{52.9}}±0.2 & {{47.0}}±0.0 & {{68.1}} \\
%  \textbf{Ours + SWAD} & \textbf{{88.4}}±0.1 & \textbf{79.6}±0.1 & \textbf{72.5}±0.2 & \textbf{53.0}±0.7 & \textbf{47.3}±0.1 &  \textbf{68.2} \\ 
% % & +0.0 & +0.0 & \blue{+0.1} & \blue{+0.1} & \blue{+0.3} & \blue{+0.1} \\
% \hline
% & \multicolumn{6}{c}{Use RegNetY-16GF~\citep{singh2022revisiting} as oracle model.} \\ 
% % MIRO  & \textbf{97.4}±0.2 & 79.9±0.6 & 80.4±0.2 & 58.9±1.3 & 53.8±0.1 & 74.1 \\
% % \textbf{Ours} & 97.3±0.1 & \textbf{82.4}±0.6 & \textbf{80.8}±0.6 & \textbf{60.7}±1.8 & \textbf{54.6}±0.1 & \textbf{75.1} \\ \hline
% % & -0.1 & \blue{+2.5} & \blue{+0.4} & \blue{+1.8} & \blue{+0.8} & \blue{+1.1} \\
% MIRO + SWAD  & 96.8±0.2 & 81.7±0.1 & 83.3±0.1 & {{64.3}}±0.3 & 60.7±0.0 & 77.3 \\
% \textbf{Ours + SWAD} & \textbf{{97.9}}±0.3 & \textbf{{82.2}}±0.3 & \textbf{{84.7}}±0.2 & \textbf{65.0}±0.2 & \textbf{{61.3}}±0.2 & \textbf{78.2} \\ 
% % & \blue{+1.1} & \blue{+0.5} & \blue{+1.4} & \blue{+0.7} & \blue{+0.6} & \blue{+0.9} \\
% \hline \hline
% % & \blue{+0.2} &  \blue{+0.1} &  \blue{+0.2} &  \blue{+0.7} &  \blue{+0.3} &   \blue{+0.3}\\ 
% % MIRO + SWAD  & \textbf{88.4}±0.1 & \textbf{\textit{79.6}}±0.2 & \textbf{\textit{72.4}}±0.1 & \textbf{\textit{52.9}}±0.2 & \textbf{\textit{47.0}}±0.0 & \textbf{\textit{68.1}} \\
% % \textbf{Ours + SWAD} & \textbf{{88.4}}±0.1 & \textbf{79.6}±0.1 & \textbf{72.5}±0.2 & \textbf{53.0}±0.7 & \textbf{47.3}±0.1 &  \textbf{68.2} \\ 
% % % & +0.0 & +0.0 & \blue{+0.1} & \blue{+0.1} & \blue{+0.3} & \blue{+0.1} \\
% % \hline
% % & \multicolumn{6}{c}{\bf Use multiple oracle models.} \\ 
% % SIMPLE & 88.6±0.4 & 79.9±0.5 & 84.6±0.5 & 57.6±0.8 & 49.2±1.1 & 72.0 \\
% % SIMPLE++ & \textbf{99.0}±0.1 & \textbf{82.7}±0.4 & \textbf{87.7}±0.4 & 59.0±0.6 & \textbf{61.9}±0.5 & \textit{\textbf{78.1}} \\ 
% %  & \multicolumn{6}{c}{\bf Use RegNetY-16GF~\citep{singh2022revisiting} as oracle model.} \\ 
% % MIRO  & 97.4±0.2 & 79.9±0.6 & 80.4±0.2 & 58.9±1.3 & 53.8±0.1 & 74.1 \\
% % \textbf{Ours} & 97.3±0.1 & 82.4±0.6 & 80.8±0.6 & 60.7±1.8 & 54.6±0.1 & 75.1 \\
% % % & -0.1 & \blue{+2.5} & \blue{+0.4} & \blue{+1.8} & \blue{+0.8} & \blue{+1.1} \\
% % MIRO + SWAD  & 96.8±0.2 & 81.7±0.1 & 83.3±0.1 & \textit{\textbf{64.3}}±0.3 & 60.7±0.0 & 77.3 \\
% % \textbf{Ours + SWAD} & \textbf{\textit{97.9}}±0.3 & \textbf{\textit{82.2}}±0.3 & \textbf{\textit{84.7}}±0.2 & \textbf{65.0}±0.2 & \textbf{\textit{61.3}}±0.2 & \textbf{78.2}
% % \\ 
% % & \blue{+1.1} & \blue{+0.5} & \blue{+1.4} & \blue{+0.7} & \blue{+0.6} & \blue{+0.9} \\
% % \hline
% \end{tabular}
% \end{center}
% \end{table*}
\textbf{Regression results: Monocular
depth estimation.}

The regression results for each unseen domain of monocular
depth estimation visualization is displayed in Figure~\ref{fig:reg_res},~\ref{fig:reg_res2}.

The Visualization of regression results for unseen domains of models trained with different objective settings are exhibited in  Figure~\ref{fig:reg_abl_res1},~\ref{fig:reg_abl_res2}.

\textbf{Segmentation results.}
The segmentation results for unseen samples are displayed in \Figref{fig:seg_res}.

\textbf{Classification results.}
We show the results of each category for the classification experiments as Table~\ref{tab:res_detial1},~\ref{tab:res_detial2},~\ref{tab:res_detial3},~\ref{tab:res_detial4},~\ref{tab:res_detial5}.
% ,,,}. 










% \begin{table*}[t]
% \caption{Cassification experiments: More results of full GMDG for each category in all benchmark datasets.}
% \label{tab:res_detial}

% \small
% \centering
%     \begin{tabular}{lccccccc}
% \\
%  \textbf{TerraIncognita} & \multicolumn{1}{c}{\textbf{Location 100}} & \multicolumn{1}{c}{\textbf{Location 38}} & \multicolumn{1}{c}{\textbf{Location 43}} & \multicolumn{1}{c}{\textbf{Location 46}} & \multicolumn{1}{c}{\textbf{Avg.}} \\ \hline
% ResNet-50 & 59.8±1.0 & 45.3±1.7 & 57.1±1.8 & 38.2±5 & 50.1±1.2 \\
% + SWAD & 61.2±1.4 & 48.4±1.6 & 60.0±0.4 & 42.5±1.1 & 53.0±0.7 \\ \hline
% RegNetY-16GF & 73.3±3.3 & 54.7±1.4 & 67.1±0.3 & 48.6±6.5 & 60.7±1.8 \\
% + SWAD & 74.3±1.5 & 59.2±1.2 & 70.6±1.1 & 56.0±0.8 & 65.0±0.2 \\ \hline \\
% \\
% \textbf{OfficeHome} & \multicolumn{1}{c}{\textbf{art}} & \multicolumn{1}{c}{\textbf{clipart}} & \multicolumn{1}{c}{\textbf{product}} & \multicolumn{1}{c}{\textbf{real}} & \multicolumn{1}{c}{\textbf{Avg.}} \\ \hline
% ResNet-50 & 68.9±0.3 & 56.2±1.7 & 79.9±0.6 & 82.0±0.4 & 70.7±0.2 \\
% + SWAD & 68.9±0.6 & 58.2±0.6 & 80.4±0.3 & 82.6±0.4 & 72.5±0.2 \\ \hline
% RegNetY-16GF & 79.7±1.6 & 67.7±1.8 & 87.8±0.8 & 87.9±0.7 & 80.8±0.6 \\
% + SWAD & 84.1±0.2 & 74.3±0.9 & 89.9±0.4 & 90.6±0.1 & 84.7±0.2 \\ \hline \\
% \\
% \textbf{VLCS} & \multicolumn{1}{c}{\textbf{caltech101}} & \multicolumn{1}{c}{\textbf{labelme}} & \multicolumn{1}{c}{\textbf{sun09}} & \multicolumn{1}{c}{\textbf{voc2007}} & \multicolumn{1}{c}{\textbf{Avg.}} \\ \hline
% ResNet-50 & 98.3±0.4 & 65.9±1 & 73.4±0.8 & 79.3±1.3 & 79.2±0.3 \\
% + SWAD & 98.9±0.4 & 63.6±0.2 & 76.4±0.5 & 79.5±0.6 & 79.6±0.1 \\ \hline
% RegNetY-16GF & 97.9±1.3 & 66.8±2.1 & 80.8±1 & 83.9±1.8 & 82.4±0.6 \\
%  + SWAD & 98.4±0.1 & 65.5±1.4 & 79.9±0.4 & 84.9±0.9 & 82.2±0.3 \\  \hline \\
% \\
% \textbf{PACS} & \multicolumn{1}{c}{\textbf{art\_painting}} & \multicolumn{1}{c}{\textbf{cartoon}} & \multicolumn{1}{c}{\textbf{photo}} & \multicolumn{1}{c}{\textbf{sketch}} & \multicolumn{1}{c}{\textbf{Avg.}} \\ \hline
% ResNet-50 & 90.1±0.6 & 83.9±0.2 & 97.6±0.5 & 82.3±0.7 & 88.4±0.1 \\
% + SWAD & 84.7±1.0 & 81.7±2.4 & 97.5±0.4 & 80.5±1.8 & 85.6±0.3 \\ \hline
% RegNetY-16GF & 97.5±1.0 & 97.0±0.2 & 99.4±0.2 & 95.2±0.4 & 97.3±0.1 \\
%  + SWAD & 98.3±0.3 & 98.0±0.1 & 99.5±0.3 & 95.3±0.8 & 97.9±0.0 \\   \hline \\
% % \end{tabular}
% % \centering
% % \begin{tabular}{llllllll}
% \\
% \textbf{DomainNet} & \multicolumn{1}{c}{\textbf{clipart}} & \multicolumn{1}{c}{\textbf{info}} & \multicolumn{1}{c}{\textbf{painting}} & \multicolumn{1}{c}{\textbf{quickdraw}} & \multicolumn{1}{c}{\textbf{real}} & \multicolumn{1}{c}{\textbf{sketch}} & \multicolumn{1}{c}{\textbf{Avg.}} \\ \hline
% ResNet-50 & 63.4±0.3 & 22.4±0.4 & 51.4±0.4 & 13.4±0.8 & 64.4±0.3 & 52.4±0.4 & 44.6±0.1 \\ 
% + SWAD & 66.4±0.3 & 23.8±0.1 & 54.5±0.3 & 15.8±0.1 & 67.5±0.1 & 55.8±0.0 & 47.3±0.1 \\ \hline
% RegNetY-16GF & 74.0±0.3 & 39.5±1.5 & 61.5±0.3 & 16.3±1.2 & 73.9±1.5 & 62.8±2.4 & 54.6±0.1 \\
% + SWAD & 79.0±0.0 & 46.9±0.4 & 69.9±0.4 & 20.7±0.6 & 81.1±0.3 & 70.3±0.4 & 61.3±0.2 \\ \hline \\
% \end{tabular}

% \end{table*}
% \end{@twocolumnfalse}
% ]


\subsection{Other findings and Analysis}
\label{app:other_findings}
\textbf{What makes a better $\mathcal{O}$.}
    % As indicated in Eq.~\ref{eq:PUB}, $\mathcal{O}$ is significant for PUB as it anchors a space where the relationship between $\rmX, \rmY$ is well preserved. Ideally, the $\mathcal{O}$ that provides the general representations of all seen and unseen domains will lead to the best results. This finding is validated in MIRO and SIMPLE. 
    % However, 
    % even though SIMPLE++ composes 283 pre-trained models, the `perfect' $\mathcal{O}$ is still not certified. 
    % Therefore, this paper mainly discusses that the model performs better with our proposed objectives when the $\mathcal{O}$ is given and fixed.  
    As demonstrated in Eq.~\ref{eq:PUB}, $\mathcal{O}$ plays a crucial role in PUB by anchoring a space where the relationship between $\rmX$ and $\rmY$ is preserved. Ideally, having one $\mathcal{O}$ that provides general representations for all seen and unseen domains leads to the best results, one finding supported by MIRO and SIMPLE. However, even though SIMPLE++ combines 283 pre-trained models, achieving the `perfect' $\mathcal{O}$ remains unattained. Therefore, this paper primarily discusses how our proposed objectives can improve the model performance when a fixed $\mathcal{O}$ is provided.
% \begin{align}
%     \min_{\phi,{\psi}}H(P ({ \phi(\rmX) , {\psi(\rmY)}})) { - H(P(\phi(\rmX)  \mid  \psi(\rmY))) -H(\mathbb{E}[ P ({\phi(\rmX_n)})]) + {H(P(\phi(\rmX)))}}. 
% \end{align}

\textbf{Comparison with MDA: Minimizing domain gap compared to the decision gap.} 
MDA~\citep{hu2020domain}, guided by the hypothesis ``guaranteed generalization only when the decision gap exceeds the domain gap", aims to minimize the ratio between the domain gap and the decision gap. This approach facilitates learning $\mathcal{D}$-independent conditional features, enhancing class separability across domains.
As Table~\ref{tab:summary} illustrates, MDA's \textbf{Reg2} objective can also be interpreted as suppressing invalid causality, aligning with our approach.
However, MDA's implementation requires manual selection of $\phi(\rmX)$ from the same $\rmY$ without using $\psi$ and \textbf{GReg2}. Our method further relaxes MDA's assumption, extending the application of the objective and making it also applicable to tasks besides classification, such as segmentation.  

\textbf{Cutting off causality form $\phi(\rmX) \to \psi(\rmY)$ may lead to collapse of the model.} We have tried to reversely suppress the causality form $\phi(\rmX) \to \psi(\rmY)$ instead of causality form $\psi(\rmY) \to \phi(\rmX)$ for monocular depth estimation in VA-DepthNet and it causes collapse. 




\textbf{{Suppressing invalid causality:}}
\textbf{{Why this design:}}
Our GMDG introduces a mapping $\psi$ for $\rmY$ to relax the static assumption, corroborating more general and practical scenarios. %However, 
Our empirical findings, as shown in
\cref{fig:GReg2}, %shows that 
reveal that
introducing 
$\psi(\rmY)$ without any constraints may not guarantee a clear decision margin for classification. 
Upon examining our objective in Eq.8 in the main manuscript, we hypothesize that %we conjecture it may be caused by 
the effect might result from
`$\psi(\rmY)$ causing $\phi(\rmX)$', which we term `invalid causality'. 
%The suppressing invalid causality term (denoted as \textbf{GReg2})
% is essentially
Thus, we designed a term to suppress such invalid causality. %suppressing invalid causality which 
This term is derived from the prediction perspective wherein $\rmY$ should be only predicted from $\phi(\rmX)$; hence, $\phi(\rmX)$ 
should not be caused by $\psi(\rmY)$. 
Consider the scenario wherein $\rmY$ and $\psi(\rmY)$ are absent during prediction - the hypothesized causality from $\psi(\rmY)$ to $\phi(\rmX)$ would disrupt the causal chain, resulting in an `incomplete' representation of $\phi(\rmX)$ then prediction degradation. 
%If $\psi(\rmY)$ causes $\phi(\rmX)$, during the prediction where $\rmY, \psi(\rmY)$ are missing, the whole causal path misses $\psi(\rmY)$ and results in `incomplete' $\phi(\rmX)$ then prediction degradation.
Hence, it is critical to suppress  $\psi(\rmY) \!\!\!\to\!\!\! \phi(\rmX)$ that may occur during joint training. Notably, the suppression is not symmetric and promotes $\phi(\rmX) \!\!\to\!\! \rmY$.
% should only be caused by $\rmX$ (??,$\phi(\rmX)$ is domain invariant term. Y is not static, $\rmY$ and $\rmX$ are synergistically caused by $\phi(\rmX)$,  $\psi(\rmY)$ is missing, then.... ). If $\rmX$ and $\psi(\rmY)$ synergistically cause $\phi(\rmX)$: $(\rmX, \psi(\rmY)) \!\!\to\!\! \phi(\rmX)$
% $\delta(\rmX, \psi(\rmY)) \!\!\to\!\! \phi(\rmX)$ where $\delta$ denotes the causal-effect function,
% the overafll causality from the combination of $\rmX$ and $\psi(\rmY)$ to $\phi(\rmX)$ is decomposed as: $\delta(\rmX, \psi(\rmY)) \!\!\to\!\! \phi(\rmX) \!\!=\!\! (\delta(\rmX \!\!\to\!\! \phi(\rmX)) \!+\! \delta(\psi(\rmY) \!\!\to\!\! \phi(\rmX)) \!+\! \eta)$ where $\eta > 0$ denotes the synergistic source interaction and  $\delta$ represents the causal-effect function. 
% In this case, 
% during the prediction where $\rmY, \psi(\rmY)$ is missing, the whole causal path misses $\psi(\rmY)$ and results in `incomplete' $\phi(\rmX)$ then prediction degradation. Hence, we need to suppress the $\psi(\rmY) \!\!\!\to\!\!\! \phi(\rmX)$ that may happen during the joint training. Notably, the suppression is not symmetric and promotes $\phi(\rmX) \!\!\to\!\! \rmY$.
\textbf{{Intuition:}} 
Intuitively, \textbf{GReg2} further `erases' the redundant information in $\phi(\rmX)$ that may be caused by $\phi(\rmY)$, which aims to refine the latent space, yielding 
better invariant latent features for predicting $\rmY$ (i.e., larger decision margin for the unseen domain as highlighted in \cref{fig:GReg2}). 


% \vspace{-0.1cm}
\begin{figure*}[ht]
  \centering
    \includegraphics[width=0.8\linewidth]{GReg2_examples.pdf}
   \caption{T-SNE map of latent features from classification models that were trained without and with \textbf{GReg2}.}
   \label{fig:GReg2}
\end{figure*}

\textbf{{GMDG's Efficiency:}}
We have analyzed the efficiency of GMDG in \cref{tab:flop_param}. Though theoretically superior in generality, GMGD may increase computational costs during training due to additional loss functions and VAE encoders. However, these auxiliary components are discarded in the inference stage, ensuring their efficiency remains unaffected. 
% ensuring that inference efficiency remains unaffected. 
% We also recognize the potential for further optimization of GMDG's architecture. 
Our confidence in the model's amenability to efficiency enhancement through careful 
% module 
design is high, and such pursuits remain a promising avenue for future work.
 %Moreover, we believe that with meticulous design of each module, the efficiency of GMDG can be significantly enhanced.  We will leave such exploration in the future.
 
 %As a more complete general objective, GMDG is superior in theory but it could indeed increase the computational consumption during training since it involves more losses and extra VAE encoders. 
%However, once the training is done, the extra components can be abnegated, and no extra consumption occurs during inference. Moreover, through a careful design of each module, we believe GMDG could be made more efficient. We will leave such exploration in the future. 

% Notably, the consumption of the proposed method can be significantly reduced through careful design and will be studied in the future while this paper mainly focuses on validating the efficacy of GMDG.




% such as ERM++.
%We highlight that we still exceed the current SOTA (SIMPLE) in classification.

% \vspace{-0.3cm}
\begin{table*}[t]
\centering
% \resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{l|ll|ll|ll|l}
\hline
                                 & \multicolumn{2}{l|}{Classification}          & \multicolumn{2}{l|}{Depth estimation}        & \multicolumn{2}{l|}{Segmentation}            &           \\
                                 & Training & \cellcolor[HTML]{D5D5D5}Inference & Training & \cellcolor[HTML]{D5D5D5}Inference & Training & \cellcolor[HTML]{D5D5D5}Inference &           \\ \hline
                                 & 99.16    & \cellcolor[HTML]{D5D5D5}49.58     & 584.44   & \cellcolor[HTML]{D5D5D5}573.78    & 209.97   & \cellcolor[HTML]{D5D5D5}167.34    & Baseline  \\
\multirow{-2}{*}{FLOPs (G)}      & 124.00   & \cellcolor[HTML]{D5D5D5}49.58     & 1543.90  & \cellcolor[HTML]{D5D5D5}573.78    & 449.83   & \cellcolor[HTML]{D5D5D5}167.34    & With GMDG \\ \hline
                                 & 2.94     & \cellcolor[HTML]{D5D5D5}1.47      & 64.42    & \cellcolor[HTML]{D5D5D5}64.27     & 23.13    & \cellcolor[HTML]{D5D5D5}22.54     & Baseline  \\
\multirow{-2}{*}{Parameters (M)} & 4.93     & \cellcolor[HTML]{D5D5D5}1.47      & 123.76   & \cellcolor[HTML]{D5D5D5}64.27     & 82.48    & \cellcolor[HTML]{D5D5D5}22.54     & With GMDG \\ \hline
\end{tabular}%
% }
\vspace{-0.2cm}
\caption{FLOPs and parameters of baselines without and with GMDG during training and inference.}
\label{tab:flop_param}
\end{table*}




\textbf{{Applicability, constraint, and limitations:}}
% \textbf{\blue{Applicability and constraints}} 
GMDG is specifically designed for mDG with accessible $P(\rmY)$, in which the model is trained on multiple seen domains and tested on one unseen domain. This task essentially requires learning the invariance across multi-domains for the prediction.  
% including classification, segmentation, and regression, and it requires accessibility to the $P(\rmY)$. 
When used in single-domain generalization or cases involving novel classes in the unseen domain, GMDG  may not be directly applicable, thus requiring further investigations. 
% Therefore, GMDG may be altered for single-domain generalization, and other cases such as unknown classes existing in the unseen domain. 
% \textbf{\blue{limitations}} 
Meanwhile, as a general objective,  our novel GMDG involves %a comprehensive set of 
additional modules/losses that may incur extra computational costs during training. We have discussed these aspects in our main paper, and we would like to leave them as future work.




% \end{page*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{reg_commercial.pdf}
    ~\\~\\
    \includegraphics[width=\linewidth]{reg_home.pdf}
    \caption{Regression results: Monocular depth estimation results between VA-Depth and our GMDG on samples from unseen domains. It can be seen that better generalization across domains is obtained with GMDG.}
    \label{fig:reg_res}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{reg_office.pdf}
    ~\\~\\
    \includegraphics[width=\linewidth]{reg_school.pdf}
    % \caption{Segmentation results visualization between RobostNet and ours on Cityscapes (unseen domain).}
    \caption{Regression results: Monocular depth estimation results between VA-Depth and our GMDG on samples from unseen domains. It can be seen that better generalization across domains is obtained with GMDG, continues.}
    \label{fig:reg_res2}
\end{figure*}



\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{ablation_vis_2.pdf}
    \caption{Regression results: Monocular depth estimation results for unseen domains of models trained with different objective settings. It can be seen that with the whole GMDG, the model performs the best generalization for all unseen domain settings.  }
    \label{fig:reg_abl_res1}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{ablation_vis_1.pdf}
    \caption{Regression results: Monocular depth estimation results for unseen domains of models trained with different objective settings, continues. It can be seen that with the whole GMDG, the model performs the best generalization for all unseen domain settings.}
    \label{fig:reg_abl_res2}
\end{figure*}



\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{SegRes.pdf}
    % \caption{Segmentation results visualization between RobostNet and ours on Cityscapes (unseen domain).}
    \caption{Segmentation results: Visualizations between RobostNet and our GMDG on samples from unseen domains. It can be seen that better generalization is obtained with GMDG.}
    \label{fig:seg_res}
\end{figure*}


\begin{table*}[t]
\small
\centering
\begin{tabular}{l|cccc|c}
\toprule
 \textbf{TerraIncognita} & \multicolumn{1}{c}{\textbf{Location 100}} & \multicolumn{1}{c}{\textbf{Location 38}} & \multicolumn{1}{c}{\textbf{Location 43}} & \multicolumn{1}{c|}{\textbf{Location 46}} & \multicolumn{1}{c}{\textbf{Avg.}} \\ \midrule
ERM~\cite{gulrajani2020search} & 54.3 & 42.5 & 55.6 & {38.8} & 47.8\\
MIRO~\cite{cha2022miro} (use ResNet-50) & - & -&- &- &{50.4} \\
\rowcolor{mygray}\textbf{GMDG} (use ResNet-50) & {59.8±1.0} & {45.3±1.7} & {57.1±1.8} & 38.2±5 & 50.1±1.2 \\ 
\midrule
ERM + SWAD~\cite{cha2021swad} & 55.4 & 44.9 & 59.7 & 39.9 & 50.0 \\
DIWA~\cite{rame2022diverse} & 57.2&  {50.1} & {60.3} & 39.8 & 51.9 \\
MIRO~\cite{cha2022miro} + SWAD~\cite{cha2021swad}   (use ResNet-50) & - & -&- &- &52.9 \\
\rowcolor{mygray}\textbf{GMDG} + SWAD (use ResNet-50)& {61.2±1.4} & 48.4±1.6 & 60.0±0.4 & {42.5±1.1} & {53.0±0.7} \\ \midrule
MIRO~\cite{cha2022miro}  (use RegNetY-16GF) & - & -&- &- &58.9 \\
\rowcolor{mygray}\textbf{GMDG} (use RegNetY-16GF) & 73.3±3.3 & 54.7±1.4 & 67.1±0.3 & 48.6±6.5 & 60.7±1.8 \\ \midrule
MIRO~\cite{cha2022miro} + SWAD~\cite{cha2021swad}  (use RegNetY-16GF) & - & -&- &- &64.3 \\
\rowcolor{mygray}\textbf{GMDG} + SWAD (use RegNetY-16GF)& \textbf{74.3±1.5} & \textbf{59.2±1.2} & \textbf{70.6±1.1} & \textbf{56.0±0.8} & \textbf{65.0±0.2} \\ 
\bottomrule
\end{tabular}
\caption{Classification experiments on TerraIncognita: More results of full GMDG for each category.}
\label{tab:res_detial1}
\end{table*}


\begin{table*}[t]
\small
\centering
\begin{tabular}{l|cccc|c}
\toprule
 \textbf{OfficeHome} & \multicolumn{1}{c}{\textbf{art}} & \multicolumn{1}{c}{\textbf{clipart}} & \multicolumn{1}{c}{\textbf{product}} & \multicolumn{1}{c}{\textbf{real}} & \multicolumn{1}{c}{\textbf{Avg.}}  \\ \midrule
ERM~\cite{gulrajani2020search} & 63.1 & 51.9  & 77.2&  78.1& 67.6\\
MIRO~\cite{cha2022miro} (use ResNet-50) & - & -&- &- &70.5±0.4 \\
\rowcolor{mygray}\textbf{GMDG} (use ResNet-50) & 68.9±0.3 & 56.2±1.7 & 79.9±0.6 & 82.0±0.4 & 70.7±0.2  \\
\midrule
ERM + SWAD~\cite{cha2021swad} &66.1 &57.7 &78.4 &80.2& 70.6 \\
DIWA~\cite{rame2022diverse} & 69.2 & 59 & 81.7& 82.2 &72.8 \\
MIRO~\cite{cha2022miro} + SWAD~\cite{cha2021swad}   (use ResNet-50) & - & -&- &- &72.4±0.1 \\
\rowcolor{mygray}\textbf{GMDG} + SWAD (use ResNet-50)& 68.9±0.6 & 58.2±0.6 & 80.4±0.3 & 82.6±0.4 & 72.5±0.2 \\ \midrule
MIRO~\cite{cha2022miro}  (use RegNetY-16GF) & - & -&- &- & 80.4±0.2 \\
\rowcolor{mygray}\textbf{GMDG} (use RegNetY-16GF) & 79.7±1.6 & 67.7±1.8 & 87.8±0.8 & 87.9±0.7 & 80.8±0.6 \\ \midrule
MIRO~\cite{cha2022miro} + SWAD~\cite{cha2021swad}  (use RegNetY-16GF) & - & -&- &- &83.3±0.1 \\
\rowcolor{mygray}\textbf{GMDG} + SWAD (use RegNetY-16GF)& \textbf{84.1±0.2} & \textbf{74.3±0.9} & \textbf{89.9±0.4} & \textbf{90.6±0.1} & \textbf{84.7±0.2} \\ 
\bottomrule
\end{tabular}
\caption{Classification experiments on OfficeHome: More results of full GMDG for each category.}
\label{tab:res_detial2}
\end{table*}

\begin{table*}[t]
\small
\centering
\begin{tabular}{l|cccc|c}
\toprule
\textbf{VLCS} & \multicolumn{1}{c}{\textbf{caltech101}} & \multicolumn{1}{c}{\textbf{labelme}} & \multicolumn{1}{c}{\textbf{sun09}} & \multicolumn{1}{c|}{\textbf{voc2007}} & \multicolumn{1}{c}{\textbf{Avg.}}\\ \midrule
ERM~\cite{gulrajani2020search}& 97.7 &64.3& 73.4 &74.6 &77.3\\
MIRO~\cite{cha2022miro} (use ResNet-50) & - & -&- &- & 79.0±0.0 \\
\rowcolor{mygray}\textbf{GMDG} (use ResNet-50)& 98.3±0.4 & 65.9±1 & 73.4±0.8 & 79.3±1.3 & 79.2±0.3\\
\midrule
ERM + SWAD~\cite{cha2021swad}&98.8& 63.3& 75.3 &79.2& 79.1\\
DIWA~\cite{rame2022diverse}&98.9& 62.4 &73.9 &78.9 &78.6 \\
MIRO~\cite{cha2022miro} + SWAD~\cite{cha2021swad}(use ResNet-50) & - & -&- &- &  79.6±0.2\\
\rowcolor{mygray}\textbf{GMDG} + SWAD (use ResNet-50) & 98.9±0.4 & 63.6±0.2 & 76.4±0.5 & 79.5±0.6 & 79.6±0.1 \\ \midrule
MIRO~\cite{cha2022miro}  (use RegNetY-16GF) & - & -&- &- & 79.9±0.6\\
\rowcolor{mygray}\textbf{GMDG} (use RegNetY-16GF) & 97.9±1.3 & \textbf{66.8±2.1} & \textbf{80.8±1} & 83.9±1.8 & \textbf{82.4±0.6} 
\\ \midrule
MIRO~\cite{cha2022miro} + SWAD~\cite{cha2021swad}  (use RegNetY-16GF) & - & -&- &- & 81.7±0.1\\
\rowcolor{mygray}\textbf{GMDG} + SWAD (use RegNetY-16GF)  & \textbf{98.4±0.1} & 65.5±1.4 & 79.9±0.4 & \textbf{84.9±0.9} & 82.2±0.3\\ 
\bottomrule
\end{tabular}
\caption{Classification experiments on VLCS: More results of full GMDG for each category.}
\label{tab:res_detial3}
\end{table*}

\begin{table*}[t]
\small
\centering
\begin{tabular}{l|cccc|c}
\toprule
 \textbf{PACS} & \multicolumn{1}{c}{\textbf{art\_painting}} & \multicolumn{1}{c}{\textbf{cartoon}} & \multicolumn{1}{c}{\textbf{photo}} & \multicolumn{1}{c|}{\textbf{sketch}} & \multicolumn{1}{c}{\textbf{Avg.}}  \\ \midrule
ERM~\cite{gulrajani2020search}  &84.7 & 80.8 & 97.2 & 79.3  &84.2\\
MIRO~\cite{cha2022miro} (use ResNet-50)& - & -&- &- & 85.4±0.4 \\
\rowcolor{mygray}\textbf{GMDG} (use ResNet-50) & 84.7±1.0 & 81.7±2.4 & 97.5±0.4 & 80.5±1.8 & 85.6±0.3\\
\midrule
ERM + SWAD~\cite{cha2021swad} &89.3 &83.4& 97.3& 82.5 &88.1\\
DIWA~\cite{rame2022diverse} &90.6 &83.4 &98.2 &83.8 &89.0\\
MIRO~\cite{cha2022miro} + SWAD~\cite{cha2021swad}   (use ResNet-50) & - & -&- &- & 88.4±0.1 \\
\rowcolor{mygray}\textbf{GMDG} + SWAD (use ResNet-50) & 90.1±0.6 & 83.9±0.2 & 97.6±0.5 & 82.3±0.7 & 88.4±0.1 \\ \midrule
MIRO~\cite{cha2022miro}  (use RegNetY-16GF)& - & -&- &- & 97.4±0.2\\
\rowcolor{mygray}\textbf{GMDG} (use RegNetY-16GF) & 97.5±1.0 & 97.0±0.2 & 99.4±0.2 & 95.2±0.4 & 97.3±0.1
\\ \midrule
MIRO~\cite{cha2022miro} + SWAD~\cite{cha2021swad}  (use RegNetY-16GF) & - & -&- &- &96.8±0.2 \\
\rowcolor{mygray}\textbf{GMDG} + SWAD (use RegNetY-16GF) & \textbf{98.3±0.3} & \textbf{98.0±0.1} & \textbf{99.5±0.3} & \textbf{95.3±0.8} & \textbf{97.9±0.0}\\ 
\bottomrule
\end{tabular}
\caption{Classification experiments on PACS: More results of full GMDG for each category.}
\label{tab:res_detial4}
\end{table*}


\begin{table*}[t]
\small
\centering
\begin{tabular}{l|cccccc|c}
\toprule
 \textbf{DomainNet} &  \multicolumn{1}{c}{\textbf{clipart}} & \multicolumn{1}{c}{\textbf{info}} & \multicolumn{1}{c}{\textbf{painting}} & \multicolumn{1}{c}{\textbf{quickdraw}} & \multicolumn{1}{c}{\textbf{real}} & \multicolumn{1}{c|}{\textbf{sketch}} & \multicolumn{1}{c}{\textbf{Avg.}} \\ \midrule
ERM~\cite{gulrajani2020search}&50.1 &63.0& 21.2 &63.7& 13.9& 52.9 &44.0 \\
MIRO~\cite{cha2022miro} (use ResNet-50)& - & -&- &- & - & -& 44.3±0.2\\
\rowcolor{mygray}\textbf{GMDG} (use ResNet-50) & 63.4±0.3 & 22.4±0.4 & 51.4±0.4 & 13.4±0.8 & 64.4±0.3 & 52.4±0.4 & 44.6±0.1 \\
\midrule
ERM + SWAD~\cite{cha2021swad} &53.5 &66.0& 22.4 &65.8& 16.1 &55.5 &46.5\\
DIWA~\cite{rame2022diverse} &55.4 &66.2& 23.3 &68.7& 16.5 &56.0 &47.7\\
MIRO~\cite{cha2022miro} + SWAD~\cite{cha2021swad}   (use ResNet-50)   & - & -&- &- & - & -&47.0±0.0\\
\rowcolor{mygray}\textbf{GMDG} + SWAD (use ResNet-50)  & 66.4±0.3 & 23.8±0.1 & 54.5±0.3 & 15.8±0.1 & 67.5±0.1 & 55.8±0.0 & 47.3±0.1\\ \midrule
MIRO~\cite{cha2022miro}  (use RegNetY-16GF) & - & -&- &- & - & -& 53.8±0.1\\
\rowcolor{mygray}\textbf{GMDG} (use RegNetY-16GF) & 74.0±0.3 & 39.5±1.5 & 61.5±0.3 & 16.3±1.2 & 73.9±1.5 & 62.8±2.4 & 54.6±0.1 
\\ \midrule
MIRO~\cite{cha2022miro} + SWAD~\cite{cha2021swad}  (use RegNetY-16GF) & - & -&- &- & - & -& 60.7±0.0 \\
\rowcolor{mygray}\textbf{GMDG} + SWAD (use RegNetY-16GF)  & \textbf{79.0±0.0} & \textbf{46.9±0.4} & \textbf{69.9±0.4} & \textbf{20.7±0.6} & \textbf{81.1±0.3} & \textbf{70.3±0.4} & \textbf{61.3±0.2}  \\ 
\bottomrule
\end{tabular}
\caption{Classification experiments on DomainNet: More results of full GMDG for each category.}
\label{tab:res_detial5}
\end{table*}






